Chaos persists in large-scale multi-agent learning despite adaptive learning rates

Multi-agent learning is intrinsically harder, more unstable and unpredictable than single agent optimization. For this reason, numerous specialized heuristics and techniques have been designed towards the goal of achieving convergence to equilibria in self-play. One such celebrated approach is the use of dynamically adaptive learning rates. Although such techniques are known to allow for improved convergence guarantees in small games, it has been much harder to analyze them in more relevant settings with large populations of agents. These settings are particularly hard as recent work has established that learning with fixed rates will become chaotic given large enough populations.In this work, we show that chaos persists in large population congestion games despite using adaptive learning rates even for the ubiquitous Multiplicative Weight Updates algorithm, even in the presence of only two strategies. At a technical level, due to the non-autonomous nature of the system, our approach goes beyond conventional period-three techniques Li-Yorke by studying fundamental properties of the dynamics including invariant sets, volume expansion and turbulent sets. We complement our theoretical insights with experiments showcasing that slight variations to system parameters lead to a wide variety of unpredictable behaviors.

==> Body/Intro_old.tex <==


The specific method for varying the learning rate that we are contributing is the WoLF
(“Win or Learn Fast”) principle. The essence of this method is to learn quickly when
losing, and cautiously when winning. The intuition is that a learner should adapt quickly
when it is doing more poorly than expected. When it is doing better than expected, it
should be cautious since the other players are likely to change their policy. The heart of the
algorithm is how to determine whether a player is winning or losing. For the analysis in


Win or Learn Fast (WoLF) is an extension to Infinitesimal
Gradient Ascent (IGA), where the step size of the learning
agent is reaching an infinitesimal step size ($\lim \rightarrow 0$) [4].
WoLF gives a stronger notion of convergence to a NES by
introducing separate learning rates for when the agent is
winning and when it is losing, referred to as aWIN and
aLOSE where aW IN < aLOSE. The agent is judged to
be winning if their current expected payoff is better than
playing the Nash equilibrium. This change has the effect of
the winning agent learning slower and being more “cautious”
about updating its strategy until the other agent has learned
to counter the new strategy.

% What is the problem oeo?
The unpredictability of human behavior in decision making at complex multi-agent strategic environments is a prevalent phenomenon in our everyday lives.
For example, in financial markets, despite the assumption of rational behavior among market participants, it is still impossible to predict future stock prices with certainty \cite{?}. Similarly, in other domains such as traffic flow on roads \cite{?} or data transmission in computer networks (ref [?]), past observations of latency may not always yield accurate predictions about future system performance \cite{?}. These phenomena in literature are often characterized as chaotic, owing to the absence of an underlying structure and order that would enable faithful predictions.

Unfortunately, the endeavor to formalize this intuitive understanding of chaos in a mathematical framework, specifically from a game theoretical perspective, is hindered by several roadblocks: $(i)$ the multitude of theoretical frameworks available for quantifying chaos, which makes it challenging to select an appropriate framework for a given game dynamic \cite{?} and $(ii)$ the  lack of equivalence among mathematical definitions of unpredictability, which can result paradoxically in a system being classified as chaotic under one definition, yet stable under another. \cite{?}

% Unpredictability is an everyday phenomenon when it comes to interacting with other people. Although all stock players are rational, there is no way to predict the tomorrow stock prices. When it comes to traffic in road or computer networks, observing past latencies may not always result in confident prediction about the future performance.
% We tend to characterize these phenomena chaotic because of the lack of structure and order which would allow us to make faithful predictions.


% When we try to convert this intuitive understanding of a chaos into a formal mathematical framework, from the perspective of game theory, we face several roadblocks: 1) Unpredictability under some definitions does not appear. 2) Multiple theoretical frameworks for quantifying chaos exist.



%@George...here we need something to say about shifting from algo and complexity to DS perspective in Game theory. @ Manolis: What do you mean?


While most of the games are studied nowadays from a dynamical system perspective, they fail to be unpredictable from a purely computational point of view. Indeed, if we know the dynamical system and the initial state, we can always by design predict the future states. %given the players' actions.


Critically, there does not seem to be a unique way of describing mathematically the notion of chaos. Multiple notion exist 
translating our intuitive notion of unpredicable in a formal framework.

1) Volume expansion:
2) Lyapunov exponents:
3) Li-yorke chaos:
4) Horseshoes and turbulent sets:
5) Existence of period of arbritrary degree:
6) Non-Ergodicity
7) Entropy
8) Fractal dimension



In general however these properties are not equivalent.

Fortunately, for the special case of 1-dimensional autonomous dynamical systems, many variants of the aforementioned defintion of chaos are shown to be equivalent to the existence of Li-yorke chaos.
Specifically, the key results of [Li-Yorke] and [Sharkovsky 3 and infinite] establish a clear dichotomy.
\emph{Either a DS has a 3-period point and consequently is chaotic or
it has not and it is simple}

Recent works had leveraged this clear dichotomy to show Li-yorke chaotic behavior in the variety of dynamics for congestion games. [Panageas], [Route to chaos], [Forel], 

Assuming decaying learning rate is aligned with the conventional wisdom of
pointwise convergence. All these results belong to the high enough  learning and static rate regime

Unfortunately the gap between real-life chaotic behaviors in games and practice remains. The above results assume that the agents follow a fixed meta-algorith which remains unchanged regardless of the historical payoff. In other words, while the state of the employed dynamical system change, the update rule itself remain fixed. Such restricted methodology is not followed by real-life agents [??]


That being said, two central questions arise:
\begin{center}
1) Are the proofs of  a mear coincidence or an indicative for chaotic behavior in more complex games\\
\&\\
2) Even if Chaos persists in these more complex systems which notion of chaos can be proved given that they are not necessarily equivalent.
\end{center}
\end{comment}


==> output/Body/Abstract.tex <==
%----------------------------------------------------------------------
%%% ABSTRACT
%----------------------------------------------------------------------
% !TEX root = ../main_new.tex
%
%
% What is the (important) problem
% MWU, game dynamics learning rate, chaotic behavior  
% Existing approaches fail
% Our solutions solves the problem
%Chaotic behaviors are observed in real life games even in conventionally easy classes like congestion games \cite{arthur1994inductive}. This behavior has been formally verified for the widely popular meta-algorithm Multiplicative Weight Updates (MWU) when agents are using high learning rates. From a behavioral perspective, there is still a large gap between these theoretical results and real life agents that can adapt their meta-behavior dynamically in response to history of the game. In this paper we aim to close this gap by extending prior results to settings where agents can dynamically change their learning rate based on a summary of the historical payoffs. At a technical level, to the best of our knowledge our results are the first to establish the existence of chaos in MWU dynamics in dynamic learning rate environments.
%with the goal of having optimal performance in the presence of stationary opponents as well a
%where the agents  can  
%learn quickly when they perform poorly and are more cautious when they are performing well.  

Multi-agent learning is intrinsically harder, more unstable and unpredictable than single agent optimization. For this reason, numerous specialized heuristics and techniques have been designed towards the goal of
achieving convergence to equilibria in self-play. One such celebrated approach is the use of  dynamically adaptive learning rates. 
Although such techniques are known to allow for
improved convergence guarantees in small 
%(two agent, two strategy)
games, it has been much harder to analyze them in more relevant settings with large populations of agents. These settings are particularly hard as recent work has established that learning with fixed  rates will become chaotic given large enough populations.
%~\cite{chotibut2019route,bielawski2021follow}.
In this work, we rigorously show that topological chaos persists in large population congestion games
despite using adaptive learning rates even for the ubiquitous Multiplicative Weight Updates (MWU) algorithm, even 
in the presence of only two strategies. The non-autonomous nature of the system under study calls for fundamentally different techniques from those used in the autonomous case, with our approach focusing on the geometric properties of the dynamics, including the investigation of invariant sets, volume expansion, and turbulent sets. We close the study discussing the attractors of the system and the asymptotic relationship between the adaptive and standard MWU algorithms. The results established in this work motivate the extension of rigorous chaos analysis to other non-autonomous multi-agent learning settings as well.



%At a technical level, due to the non-autonomous nature of the system, our approach goes beyond conventional period-three techniques
 %~\cite{liyorke} 
 %by studying  fundamental properties of the dynamics including 
%invariant sets, volume expansion and turbulent sets. 
%We complement our theoretical insights with experiments showcasing that slight variations to system parameters lead to a wide variety of unpredictable behaviors.

%as they result in non-autonomous dynamical systems which are notoriously hard to formally argue about .
%Intuitively, the problem is that the whole population gets locked-in a regime where every agent is dissatisfied and thus try to learn with a large learning rate. Unfortunately, 
 %period-two orbits, 

%Interactions and behaviors observed in real-world games can often exhibit a degree of unpredictability, as exemplified by the difficulty in predicting today's traffic  based on yesterday's observations. Game theory offers a framework for formalizing such intuitive statements, through the concept of Li-Yorke chaos. Specifically, standard meta-algorithms like Multiplicative Weight Updates (MWU) are shown to be Li-Yorke chaotic for congestion games when agents show volatile behavior via increased learning rates. Yet these results still fall short of capturing the full complexity of real life behavior by assuming that the agent meta-behavior remains static irrespective of the historical payoffs. This limitation allows for a formal proof of chaos through the demonstration of a 3-period cycle in these dynamics. In this work, we aim to close the gap between theory and practice by formally proving the existence of Li-Yorke chaos in a class of games where agents can adaptively change their learning rates based on a summary of historical payoffs. At a technical level, our approach goes beyond conventional period-three techniques by studying  fundamental properties of the dynamics including 
%period-two orbits, invariant sets, 
%volume expansion and turbulent sets.       


==> output/Body/Discussion.tex <==
%----------------------------------------------------------------------
%%% INTRODUCTION
%----------------------------------------------------------------------
% !TEX root = ../main_new.tex


%This is the introduction, and this is a test citation of \citet{Nas51}.


We have formally analyzed and established chaotic behavior for a class of multi-agent learning systems with a heuristically updated, variable learning rate. Interestingly, the resulting system is non-autonomous, requiring substantial departures from prior approaches to establishing Li--Yorke chaos in games, such as the celebrated period-3 methodology~\cite{liyorke}, which relies on repeated iterations of a fixed, time-invariant map and is therefore not directly applicable in the present setting.
%To do so, we were inspired by intuition and modelling decisions based on classic AI works in the area such as~\citet{bowling2002multiagent,bowling2004convergence} while simultaneously extending deep technical insights about Li-Yorke chaos in games, which has received a lot of attention recently, popping up in numerous application areas from congestion games \cite{palaiopanos2017multiplicative,chotibut2019route,bielawski2021follow}, to market economies \cite{cheung2021learning}, blockchain mechanism design \cite{leonardos2021dynamical} and even performative prediction~\cite{piliouras2022multi}.
%At the technical crux of all prior formal analysis of Li-Yorke chaos in games (e.g., \cite{bielawski2021follow,chotibut2019route,leonardos2021dynamical,cheung2021learning,piliouras2022multi})  lied the 
%celebrated methodology based on period three orbits~\cite{liyorke}, which is only applicable in autonomous, i.e., time-invariant systems.
In contrast, our analysis requires a deeper examination of the geometry and structural properties of the dynamics, which themselves evolve over time. Nevertheless, we show that a rigorous analysis of chaotic behavior remains possible in this setting. This opens the door to extending existing results to more realistic time-varying models and to establishing rigorous notions of chaos in such systems as well.

%One natural direction for future work is to study to what extent such techniques can be applied in the other application areas encountered above, e.g., to better understand the evolution of markets and blockchain mechanisms under volatility of their exogenous parameters. Another exciting direction is to explore different classes of multi-agent based systems with a variable learning rate, e.g., based on Follow-the-Regularized-leader dynamics~\cite{bielawski2021follow} or Proximal Policy Optimization~\cite{ratcliffe2019win}.  It would also be interesting to identify settings where our motivating question admits a positive answer, i.e., novel classes of dynamically updated learning rates which whilst allowing fast escape from non-promising regions also converge to equilibria in games with large populations of agents.


%It is well known that this technique has shown promise both theoretically and experimentally in small games and particularly in the special case of two agents, two strategy games, however . 


==> output/Body/DynamicRate.tex <==

Turning our attention to the dynamic learning rate setting, we will refer to $x_n(x_0)$  as the $n$-th iterate given the initialization $x_0$, and $a_{n}(x_0)$ the learning rate at the same iteration, respectively. In this section we prove some fundamental properties of the adaptive learning dynamics associated with the existence of a forward \& absorbing set, the convergence of the Ces\`{a}ro means, even when the dynamics is complex and the volume expansion. Particularly the latter will prove useful in the section where the learning dynamics under study will be shown to be Li--Yorke chaotic.

\subsection{Forward invariant \& absorbing set in dynamic learning rates.}
Leveraging the existence of the perpetual set $\mathcal{F}(a)$ in the fixed rate case, we can construct a forward invariant absorbing set. This set will be crucial in proving the Li--Yorke chaotic behavior for the non-autonomous case. Intuitively, although the learning rate is varying both among different initializations and iterations, there exists a set which corresponds to the closure of all perpetual sets $\{\mathcal{F}(a_n)\}$, to which our dynamics are always absorbed. This motivates the definition of set $\Delta$ as 
$$\Delta = \left[\min_{a \in [a_{\min},a_{\max}]}f_{\min}(a) , \max_{a \in [a_{\min},a_{\max}]}f_{\max}(a)\right]$$ 
where $a_{\min}$ and $a_{\max}$ are the $\inf_{r\in\mathbb{R}}g(r)$ and 
$\sup_{r\in\mathbb{R}}g(r)$, respectively. 

\begin{lemma}[Forward Invariance Property]\label{lemma:forward-dynamic}
For all $a_{\min} > s_b$ we get that  $\Delta$ is forward invariant, i.e.
\begin{align*}
x_n(x_0) \in \Delta \implies x_{n+1}(x_0) \in \Delta.
\end{align*}
\end{lemma}
\begin{proof}
We have three cases to consider. The first one 
\begin{equation*}
 x_n(x_0) \in [f_{\min}(a_n(x_0)), f_{\max}(a_n(x_0))] \implies x_{n+1}(x_0) \in [f_{\min}(a_n(x_0)), f_{\max}(a_n(x_0))]   
\end{equation*}
and the result follows trivially because of the perpetual set $\mathcal{F}(a_n(x_0))$. For the second case we get
\begin{equation*}
    x_n(x_0) \in \left[\min_{a \in [a_{\min},a_{\max}]}f_{\min}(a), f_{\min}(a_n(x_0))\right) \implies x_{n+1}(x_0) \in \left[\min_{a \in [a_{\min},a_{\max}]}f_{\min}(a), f_{\max}(a_n(x_0))\right]
\end{equation*}
and thus the result follows for this one as well. The last case is
\begin{equation*}
    x_n(x_0) \in \left(f_{\max}(a_n(x_0)), \max_{a \in [a_{\min},a_{\max}]}f_{\max}(a)\right] \implies x_{n+1}(x_0) \in \left[f_{\min}(a_n(x_0)), \max_{a \in [a_{\min},a_{\max}]}f_{\max}(a)\right]
\end{equation*}
Clearly the result holds for all cases.
\end{proof}


More interestingly, we  can show that eventually, any subinterval of $(0,1)$ will be absorbed within $\Delta$.
\begin{lemma}[Absorption Property]\label{lemma:absorption-dynamic}
For all $a_{\min} > s_b$ and $[\gamma, \zeta] \subset (0,1)$, there is an $n_0 \geq 0$ so that
\begin{align*}
      \forall n \geq n_0 \quad x_{n}([\gamma, \zeta]) \subseteq \Delta.
\end{align*}
\end{lemma}
\begin{proof}
Let us define the three following sets 
\begin{align*}
    U_0 = \left[\gamma, \min_{a \in [a_{\min},a_{\max}]}f_{\min}(a)\right) \quad 
    \Delta_0 = \Delta \cap [\gamma, \zeta] \quad 
    V_0 = \left(\max_{a \in [a_{\min},a_{\max}]}f_{\max}(a), \zeta\right]
\end{align*}
It suffices to prove the theorem for each of them (if they are non-empty) because we can pick \[n_0 = \max\{n_0(U_0), n_0(\Delta_0), n_0(V_0)\}\] (excluding any empty sets) to satisfy the theorem.
Based on Lemma~\ref{lemma:forward-dynamic}, it is clear that $n_0(\Delta_0) = 0$. Moving on to the case of $U_0$, we know that in $U_0$ we have that $f(x, a, b) > x$. We can define a uniform bound on their difference
\begin{equation*}
    \min_{x \in U_0} \min_{a \in [a_{\min},a_{\max}]} \left[ f(x, a, b) -x \right] = \xi > 0
\end{equation*}
We now know that
\begin{equation*}
    x_1(U_0) \in \left[\gamma + \xi, \max_{a \in [a_{\min},a_{\max}]}f_{\max}(a)\right)
\end{equation*}
If $x_1(U_0) \subset \Delta$ then the result follows trivially for $n_0 = 1$. Otherwise we have that
\begin{equation*}
    x_1(U_0) \in \left[\gamma + \xi, \min_{a \in [a_{\min},a_{\max}]}f_{\min}(a)\right) \subset U_0
\end{equation*}
Applying recursively, either there is a $n_0$ such that $x_{n_0}(U_0) \subset \Delta$ and the theorem holds for $U_0$ or for all $n$ we have that $x_n(U_0)$ stays in a subset of $U_0$
\begin{equation*}
    x_n(U_0) \in \left[\gamma + n\xi, \min_{a \in [a_{\min},a_{\max}]}f_{\min}(a)\right) \subset U_0
\end{equation*}
But this is impossible since there is a $n_0>0$ such that 
\begin{equation*}
 \forall n \geq n_0 : \gamma + n\xi >   \min_{a \in [a_{\min},a_{\max}]}f_{\min}(a) 
\end{equation*}
The case of $V_0$ can be handled symmetrically.
\end{proof}

We note that the key observation for the proof of both the aforementioned lemmas is the fact that at any iteration $x_n(x_0)$ will always come closer to the perpetual absorbing set $\mathcal{F}(a_n(x_0))$ and thus to its closure $\Delta$. 

An immediate consequence of this lemma is the following corollary which will be a key element for the uniform convergence both of our proposed \emph{pseudo-regret} notion and the Ces\`{a}ro mean of the iterations. Analytically, for a given subinterval $[\gamma,\zeta]$ of $(0,1)$, we can always choose some $\delta>0$ such that $\Delta\cup [\gamma,\zeta]\subseteq(\delta, 1 - \delta)$. Again such  choice of $\delta$ is possible because the attraction to $\Delta$ is not eventual phenomenon \textendash\ at each iteration, $\mathrm{dist}(x_n(x_0),\Delta)$ will be either zero or always decreasing . This argumentation is expressed by the following statement:
\begin{corollary}\label{corollary:bound}
Let $a_{\min} > s_b$, then for every $[\gamma, \zeta] \subset (0,1)$, there is an $\delta > 0$ so that
\begin{align*}
      \forall n \geq 0 \quad x_{n}([\gamma, \zeta]) \subseteq (\delta, 1 - \delta).
\end{align*}
\end{corollary}

\subsection{Uniform Convergence of Ces\`{a}ro means \& Learning Rate.}
Having established Corollary~\ref{corollary:bound}, we are now in a position to present our claims regarding the average convergence for any initialization in $(0,1)$. Notably, while the individual iterates of the system, as we shall demonstrate in the ensuing section, exhibit chaotic characteristics, the iterate averages display stabilization over time.

Corollary~\ref{corollary:bound} indicates that for any $x_0 \in (0,1)$, $x_n(x_0)$ will remain bounded away from the endpoints ${0,1}$. We now seek to connect how the boundness away from ${0,1}$ affects the average iterate of a trajectory. By induction on $x_{n+1} = f(x_n, a_n, b)$ we can prove the following 
\begin{equation}
    x_n = \frac{x_0}{x_0 + (1-x_0)\exp\left(\sum_{i=0}^{n-1} a_i(x_i-b)\right)}.\label{eq:MWU-varying}
\end{equation}
Observe that if we choose a $x_0 \in (0,1)$, then $x_n$ is bounded away from ${0,1}$ if and only if $\sum_{i=0}^{n-1} a_i(x_i-b)$ is bounded. Specifically we can prove:
\begin{lemma}\label{ref:average}
Let $a_{\min} > s_b$ and $x_0 \in (0,1)$, then
\begin{equation*}
    \lim_{n \to \infty}\frac{1}{n+1}\sum_{i=0}^n a_i(x_0)(x_i(x_0) - b) = 0.
\end{equation*}
\end{lemma}
\begin{proof}
Observe that $x_0 \in (0,1)$, so by Corollary~\ref{corollary:bound} there is a $\delta > 0$ such that $\delta < x_n < 1-\delta$. Thus we have
\begin{equation*}
    \frac{x_0}{1-\delta} < x_0 + (1-x_0)\exp\left(\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b)\right) < \frac{x_0}{\delta}
\end{equation*}
so we have that
\begin{equation*}
    \delta^2 < \frac{x_0\delta}{1-\delta} < (1-x_0)\exp\left(\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b)\right) < \frac{x_0(1-\delta)}{\delta} < \frac{1}{\delta}
\end{equation*}
Clearly we have that
\begin{equation*}
    \delta^2 < \exp\left(\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b)\right) < \frac{1}{\delta^2}
\end{equation*}
By taking the logarithm and dividing by $n$ we have
\begin{equation*}
    \frac{\ln(\delta^2)}{n} < \frac{1}{n}\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b) < - \frac{\ln(\delta^2)}{n}
\end{equation*}
By taking the limit, the result follows easily.
\end{proof}

Upon examination of the proof, a salient conclusion is that as $x_0$ moves farther away from the absorbing set $\Delta$ and closer to the endpoints ${0,1}$, the aforementioned convergence rate becomes increasingly slow, and fails in the case that $x_0\in\{0,1\}$, precluding a blanket result for the closed interval $[0,1]$. Conversely, if we restrict our attention to an arbitrary subinterval $[\gamma,\zeta]$, bounded away from the endpoints, we can always exploit the minimum convergence rate of this interval to derive a uniform convergence bound for the learning rate.

\begin{lemma}~\label{ref:uniform}
Let $a_{\min} > s_b$. The sequence of functions $a_n(\cdot)$ is converging uniformly to the constant function $a^\star(\cdot) = g(0)$ in every interval $[\gamma, \zeta] \subset (0,1)$.
\end{lemma}
\begin{proof}
By Corollary~\ref{corollary:bound} $x_0 \in [\gamma, \zeta]$ there is a $\delta>0$ such $\delta < x_n < 1-\delta$. Following the steps of Lemma~\ref{ref:average}
\begin{equation*}
    \frac{\ln(\delta^2)}{n} < \frac{1}{n}\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b) < - \frac{\ln(\delta^2)}{n}
\end{equation*}
Clearly this implies that for any $n>0$
\begin{equation*}
    a_{n}(x_0) = g\left(\frac{1}{n}\sum_{i=0}^{n-1} a_i(x_0) (x_i(x_0)-b)\right) \in g\left(\left[\frac{\ln(\delta^2)}{n}, - \frac{\ln(\delta^2)}{n}\right]\right) 
\end{equation*}
Since $g$ is continuous, for every $\epsilon>0$ there is a $n_0$ such that $\forall n \geq n_0$ we have that
\begin{equation*}
 \abs{a_n(x_0) - g(0)} \leq \epsilon.   
\end{equation*}
Uniform convergence follows immediately.
\end{proof}


Having established that $a_n(x_0)$ converges to $a^\star=g(0)$ for any $x_0\in(0,1)$, we are able to strengthen Lemma~\ref{ref:average}, demonstrating that its unweighted version of the Ces\`{a}ro mean (i.e. the average iterate in the limit of infinite time) also converges to $b$. 
\begin{lemma}\label{ref:cesaro}
Let $a_{\min} > s_b$ and $x_0 \in (0,1)$, then
\begin{equation*}
    \lim_{n \to \infty}\frac{1}{n+1}\sum_{i=0}^n x_i(x_0) = b.
\end{equation*}
\end{lemma}
\begin{proof}
Let us define $\rho_n = a_n(x_0) - a^\star$. Obviously $\lim_{n \to \infty} \rho_n = 0$. Then applying Lemma~\ref{ref:average} we have
\begin{equation*}
    0 = \lim_{n \to \infty}\frac{1}{n+1}\sum_{i=0}^n a_i(x_0)(x_i(x_0) - b) = \lim_{n \to \infty}\left[\frac{a^\star}{n+1} \sum_{i=0}^n (x_i(x_0) - b)  + \frac{1}{n+1}\sum_{i=0}^n \rho_i(x_i(x_0) - b)\right]
\end{equation*}
Clearly we have that $\lim_{n \to \infty} \rho_n (x_n(x_0) -b) = 0$ since $x_n(x_0)$ is bounded. And thus we obviously have
\begin{equation*}
    0 = \lim_{n \to \infty}\left[\frac{a^\star}{n+1} \sum_{i=0}^n (x_i(x_0) - b) \right]
\end{equation*}
Given that $a^\star$ is positive, the lemma follows.
\end{proof}
It is noteworthy that, despite this being equivalent to the guarantee provided in prior work, e.g. \cite{chotibut2019route}, for the fixed learning rate case, the machinery developed here for the adaptive rate regime has been more complex and involved.

\subsection{Uniform convergence of varying step-size MWU map and volume expansion.}
We now investigate the relationship between $(x_n(x_0),a_n(x_0))$ and the MWU map with a fixed learning rate $f(x_n(x_0),a^\star,b)$ as well as the volume expanding properties of the adaptive learning map. The proofs of the present subsection are deferred to Appendix \ref{app:lemma:dynamic-strong-convergence}. The next lemma will be essential in our proofs of chaos.

\Needspace{28\baselineskip}
\begin{lemma}\label{lemma:dynamic-strong-convergence}
Let $a_{\min}> s_b$. For every $k$, $\epsilon>0$ and $[\gamma, \zeta] \subset (0,1)$
\begin{equation*}
    \exists n_0: \forall n \geq n_0 \ \max_{x_0 \in [\gamma, \zeta]} \abs{x_{n+k}(x_0) - f^k(x_n(x_0), a^\star, b)} \leq \epsilon.
\end{equation*}
\end{lemma}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/plot_conv_x.pdf}
    \caption{Visualization of the uniform convergence described in Lemma \ref{lemma:dynamic-strong-convergence} for the particular system described in \eqref{sys_example} of Section \ref{sec:sec 6}.}
    \label{fig:dynamic-strong-convergence}
\end{figure}



We can intuitively think of this result as a form of uniform convergence result for the sequence of MWU maps with varying learning rates to the fixed learning rate map. However, as we stress in Section \ref{sec:sec 6}, this property should not be confused with an orbit of \eqref{eq:old-update} and the MWU system with $a^\star$, with the same $x_0$ converging to the same attractor. Fig. \ref{fig:dynamic-strong-convergence} illustrates Lemma \ref{lemma:dynamic-strong-convergence}, for the particular system described in \eqref{sys_example} of Section \ref{sec:sec 6}. 

We now prove two volume expansion lemmas for the dynamic learning rate case, namely that neighborhoods of $b$ within $\mathcal{D}(a_{\min})$ eventually expand to at least $\mathcal{F}(a_{\min})$. The intuition  behind this result is based on the monotonicity property of $\mathcal{F}(a)$. Specifically, for high enough learning rates $a_1\leq a_2$, we have that $\mathcal{F}(a_1)\subseteq \mathcal{F}(a_2)$. Fig. \ref{vol_exp} provides an illustration of the following lemma.

\Needspace{28\baselineskip}
\begin{lemma}\label{lemma:dynamic-learning:volume-expansion-basic}
For every $b \in (0,1)$, there is a $z_b$ such that for all $a_{\min} > z_b$ it holds that for every $[\gamma, \zeta]$  such that $\{ b\} \subset [\gamma, \zeta] \subseteq \mathcal{D}(a_{\min})=[x_{\max}(a_{\min}), x_{\min}(a_{\min})]$
\begin{equation*}
     \exists n_0: \ \forall n \geq n_0 \ \  x_{n}([\gamma, \zeta]) \supseteq %[f_{\min}(a_{\min}), f_{\max}(a_{\min})]=
     \mathcal{F}(a_{\min}).
\end{equation*}
\end{lemma}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/plot_vol_expan.pdf}
    \caption{Illustration of the volume expansion as described in Lemma \ref{lemma:dynamic-learning:volume-expansion-basic}}
    \label{vol_exp}
\end{figure}



It is worth mentioning that the series of Lemmas \ref{lemma:forward-dynamic}, \ref{lemma:absorption-dynamic}, \ref{ref:average} \ref{ref:uniform} and \ref{ref:cesaro},\ref{lemma:dynamic-learning:volume-expansion-basic} of this section \textendash pertaining to forward invariance, absorption, volume expansion, and convergence of Ces\`{a}ro means \textendash hold actually regardless of the choice of the update rule and are of independent interest. For the case of the fixed learning rate, Theorem~\ref{thm:volume-expansion} makes a more refined prediction compared to Lemma~\ref{lemma:dynamic-learning:volume-expansion-basic} as the former provides an equality. In the dynamic learning rate case there is a gap between the eventual image upper bound, $\Delta$ and the volume expansion lower bound $\mathcal{F}(a_{\min})$. In order to close this gap we will make use of the fact that the learning rate converges to $g(0)$.

Building upon the full range of the developed machinery of this section, we will strengthen the above volume expansion result  by showing that $ a_{\min}$ could be actually substituted by any $\tilde{a}=a^\star-\epsilon$ for any sufficiently small $\epsilon > 0$ such that  $a^\star-\epsilon >a_{\min} > z_b$. Our first observation is that thanks to the uniform convergence of $a_n \to a^\star$ in $[\gamma, \zeta] \subset (0,1)$ there exists a $n^{\dag}$ such that 
% \[
% \forall n \geq n^{\dag} \quad a_{n}([\gamma, \delta]) \subseteq (a^\star-\epsilon, a^\star+\epsilon)
% \]
% which implies that  there exists a $n^{\dag}$ such that
\begin{equation*}
    \forall n > n^{\dag} \quad \forall x \in [\gamma, \zeta] \quad a_n(x) > a^\star-\epsilon = \tilde{a}
\end{equation*}
This strengthens the previous volume expansion result to at least the set $\mathcal{F}(\tilde{a})$ for any $\tilde{a}$ close to $a^\star$.
\begin{theorem}\label{theorem:dynamic-volume-expansion}
For $a_{\min} > z_b$ and for any sufficiently small $\epsilon > 0$ such that  $a^\star-\epsilon >a_{\min} > z_b$ we have that for all $[\gamma, \zeta]$ such that 
$\{ b\} \subset [\gamma, \zeta] \subset (0,1)$, it holds that
\begin{equation*}
      \exists n_0: \ \forall n \geq n_0 \quad x_{n}([\gamma, \zeta]) \supseteq \mathcal{F}(a^\star-\epsilon).
\end{equation*}
\end{theorem}

In a completely similar fashion we can show that the absorbing set $\Delta$ can also be refined. For a given interval  $[\gamma, \zeta] \subset (0,1)$, as the learning rates converge to $a^\star$, the trajectories will tend to be absorbed by $\mathcal{F}(a^\star)$. Thus the dynamic learning rate volume expansion behavior matches fixed learning rate case in the long run.


==> output/Body/FixedRate.tex <==

%\begin{figure}[h!]
%\centering\includegraphics[width=0.7\textwidth]{Figures/mwu.pdf} 
%    \caption{The order of 
%    {\color{orange}$ f_{min}(a) $},
%    {\color{red}$ x_{\max}(a)$},
%    {\color{black}$ b $},
%    {\color{magenta}$ x_{\min}(a) $},
%    {\color{OliveGreen}$ f_{max}(a)$} in $x$-axis.
%    }
%    \label{fig:my_label}
%\end{figure}


We start our analysis by providing a refined analysis in the regime of fixed learning rate as in \cite{chotibut2019route}. The proofs of the technical results of the present section are deferred to Appendix \ref{app:fixed}. In the following we will examine conditions of such systems under the assumption of $a>4$. Let us study the local minima and maxima of $f$:
\begin{equation*}
    x_{\min/\max}(a) = \frac{1}{2} \pm \sqrt{\frac{1}{4} - \frac{1}{a}} %,\quad x_{\min}(a) = \frac{1}{2} + \sqrt{\frac{1}{4} - \frac{1}{a}}}
\end{equation*} 
Correspondingly we will denote $f_{\max}(a)=f(x_{\max}(a),a,b)$ and $f_{\min}(a)=f(x_{\min}(a),a,b)$. Our first observation is connected with the order of these values for high enough learning rate:
\Needspace{27\baselineskip}
\begin{lemma}\label{lemma:structure}
For every $b \in (0,1)$, there is a $a_b$ such that for all $a> a_b$
\begin{equation*}
    f_{\min}(a) < x_{\max}(a)< b < x_{\min}(a) < f_{\max}(a)
\end{equation*}
and $f_{\min}(a)$ is decreasing and  $f_{\max}(a)$ is increasing.
\end{lemma}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/plot_f.pdf}
    \caption{The order of $ f_{\min}(a) $, $ x_{\max}(a)$, $ x_{\min}(a) $ and $ f_{max}(a)$ in the $x$-axis.}
    \label{fig:my_label}
\end{figure}


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.6\textwidth]{Figures/mwu.pdf}
%     \caption{The order of 
%     {\color{orange}$ f_{min}(a) $},
%     {\color{red}$ x_{\max}(a)$},
%     {\color{black}$ b $},
%     {\color{magenta}$ x_{\min}(a) $},
%     {\color{OliveGreen}$ f_{max}(a)$} in $x$-axis.
%     }
%     \label{fig:my_label}
% \end{figure}

Illustratively, the order described in Lemma \ref{lemma:structure} is shown in Fig. \ref{fig:my_label}. Additionally, by construction, we can show that the interval 
$\mathcal{F}(a)=[f_{min}(a) , f_{max}(a)]$ is a forward invariant set for our dynamical system. 
In other words, if the MWU map with fixed learning rate $a$ starts in a state that is within $\mathcal{F}(a)$, it will remain in that set for all future times.
\begin{lemma}\label{lemma:forward}
For every $b \in (0,1)$ there is a $s_b$ such that  $\mathcal{F}(a)$ is forward invariant for all $a> s_b$, i.e. $$
    x \in \mathcal{F}(a) \Rightarrow f(x, a, b) \in \mathcal{F}(a).$$
\end{lemma}
We can also prove that $f$ is surjective on $\mathcal{F}(a)$ for high enough learning rates.
\begin{lemma}\label{lemma:perpetual}
For $a > a_b$, $f$ is surjective on $\mathcal{F}(a)$, i.e. 
$
    f(\mathcal{F}(a), a, b) = \mathcal{F}(a).
$
\end{lemma}
When $\mathcal{F}(a)$ is both surjective and forward invariant as is the case for $a> a_b, s_b$, we will call $\mathcal{F}(a)$ a \emph{perpetual} set. Actually, $\mathcal{F}(a)$ is also an absorbing set for all $x\in(0,1)$, in the following sense:

% \begin{proof}
% We already know that the right hand side is a super set of the left hand side by \Cref{lemma:forward}. But by \Cref{lemma:structure} we have that $x_{\max}(a)$ and $x_{\min}(a)$ belong to $[f_{\min}(a), f_{\max}(a)]$. So the left hand is a super set of the left hand side. Thus the result follows.
% \end{proof}  

\begin{lemma}\label{lemma:absorbption}
Let $a> s_b$,  $
      x_0 \in [\gamma, \zeta] \Rightarrow \exists n_0 : \ \forall n \geq n_0 \text{ s.t } \ x_{n} \in \mathcal{F}(a)
$,  for every $[\gamma, \zeta] \subset (0,1)$.
\end{lemma}

We now turn to the chaotic properties of $f$. Given that period-3 orbits do not carry over to the dynamic learning rate case, we choose to study an alternative property of chaotic maps, namely volume expansion. In autonomous maps, the existence of period-3 orbits together with \cref{thm:Li-Yorke} imply that there is an initialization set whose volume under the dynamics expands quickly. Intuitively, the more volume this initialization set covers the more chaotic the dynamic is. While \cref{thm:Li-Yorke} guarantees the existence of volume expansion, it does not quantify how much volume it eventually covers. We prove that any interval around $b$ is sufficient to eventually cover $\mathcal{F}(a)$:

%It is clear that as $\alpha\to\infty$, the function $f$ converges to a step-like function $f_{\infty}(x)=1$ for $x\in(0,b)$ and $f_{\infty}(x)=0$ for $x\in(b,1)$. 
% Hence the only candidate for a volume expanding neighborhood is the one around  $x=b$. To quantify the volume expansion in this neighborhood, we will use the key observation that $f$ is strictly decreasing in $\mathcal{D}=[x_{\max}(a),x_{\min}(a)]$.
% %In order to fill this gap, we begin by providing some useful insights for the case two-period trajectories, and its connection to chaos.
% % We want to make sure that there exists a set of initializations such that that cover the presented perpetual set. This is trivial for the fr since we can always use I as a set of initialization. This situation is less clear since for dynamic learning rate because of different alpha in each iteration.
% % One way to sidestep this roadblock is to prove that even small intervals eventually expands over the dynamics to cover almost all of the perpetual set.
% % Existing work has proved via 3-period lemma that neighborhood with volum expansion properties exist but they fall short of quantifying the expansion of this initialization set.
% The following fact will be useful later:
% \begin{claim}\label{claim:period-two}
% Let $g$ be a continuous decreasing function on a closed interval $I$ and that there exists a $x_0 \in I$ such that $\forall n: g^n(x_0) \in I$. Then 
% %  \begin{align*}
% %     g(\limsup_{n \to \infty} g^n(x_0)) = \liminf_{n \to \infty} g^n(x_0)\\
% %     g(\liminf_{n \to \infty} g^n(x_0)) = \limsup_{n \to \infty} g^n(x_0)
% % \end{align*}
% either $g^n(x_0)$ converges to a fixed point $x^\star$ or to a 2-period trajectory.
% \end{claim}

% Interestingly, if we restrict our attention to the interval $\mathcal{D}$, we can show that there is no 2-period trajectory:
% \begin{lemma}\label{lemma:period-two-trajectory}
% For every $b \in (0,1)$, there is a $\ell_b$ such that for all $a > \ell_b$, there is no period two trajectory for which both endpoints belong to $[x_{\max}(a), x_{\min}(a)]$.
% \end{lemma}

% % Additionally, it is easy to check that the only three fixed points for the MWU map are $\{0,b,1\}$. Recall now that in the case of a smooth dynamical system, the stability of a fixed point is determined by the value of the derivative of the function at that point, $f'(x_0)$. Specifically, if the absolute value of the derivative, $|f'(x_0)|$, is greater than 1, the fixed point is considered to be unstable (See \cite{Shub}). It is easy to check that for any choice of learning rate both pure actions are unstable, while for the case of mixed equilibrium $x=b$, there exists always a high enough regime of learning rates where this also holds:

% Additionally, it is easily verifiable that the only fixed point in $\mathcal{D}$ is $x^\star=b$. However, it is unlikely that the system will converge to $b$ starting from a neighborhood around it for high enough learning rate. The following lemma is a consequence of the Stable Manifold Theorem (See \cite{Shub})
% \begin{lemma}\label{lemma:instability_of_b}
% For every $b \in (0,1)$, there is a $k_b$ such that for $a> k_b$ it holds that
% there exists some neighborhood $ \mathcal{N}_{\delta}=(b-\delta,b+\delta)$, such that almost all initializations from $\mathcal{N}_{\delta}$ do not converge to $x^\star=b$.
% \end{lemma}

% % Therefore, if we focus on $\mathcal{D}$ neither two-period trajectories can be eventually detected nor all initialization neighborhoods of  which will converge to $b$, the unique interval point of the interval.
% Hence, combining Lemma~\ref{lemma:period-two-trajectory} and \ref{lemma:instability_of_b}, we can ensure the existence of an initialization set that escapes from $\mathcal{D}$. Actually, we are able to prove an even more general volume expansion theorem connecting any neighborhood of $b$ with the presented perpetual set $\mathcal{F}(a)$ leveraging its absorbption property (Lemma~\ref{lemma:absorbption}).
\begin{theorem}\label{thm:volume-expansion}
For every $b \in (0,1)$, there is a $v_b$ such that for all $a > v_b$ and  any interval $[\gamma, \zeta]$  : $  \{ b\} \subset [\gamma, \zeta] \subset (0,1) $, it holds that
\begin{equation*}
 \exists n_0 : \ \forall n \geq n_0 \quad f^n([\gamma, \zeta], a, b) = \mathcal{F}(a).
\end{equation*}
\end{theorem}

The proof of this theorem, which notably has not been established in any prior work, relies on a novel argument that is based on the monotonicity of $f$ on $\mathcal{D}=[x_{\max}(a), x_{\min}(a)]$, the lack of period-2 trajectories in $\mathcal{D}$ and the instability of fixed point $x=b$.

%To sum up, in this section, we manage to quantify  the eventual image of any neighborhood around $b$, which notably has not been established in any prior work.
The key takeaway for the next section is that we can focus our efforts on analyzing the behavior of the non autonomous system in the interior of $(0,1)$ with special attention to neighborhoods of $b$ that alone can exhibit chaotic behavior. This is especially important because as we will see our notion of pseudo-regret converges uniformly in closed intervals in the interior of $(0,1)$ but not on $[0,1]$.

==> output/Body/Introduction.tex <==
%----------------------------------------------------------------------
%%% INTRODUCTION
%----------------------------------------------------------------------
% !TEX root = ../main_new.tex


%This is the introduction, and this is a test citation of \citet{Nas51}.

% Here is a problem. How do MAL dynamics with variable learning rates behave in large games? How can we analyze them?
% It is an interesting problem.
% There is a lot of prior work on the ML side showing that at least in small games there are provable advantages when allowing for agents to adapt their learning rates based on cues coming from the state of the game.
% It is an unsolved problem. No positive results are known. Arguing about negative results is known to require techniques which are not applicable in our case.
% Here is our solution 
% Our solution works


Arguably one of the most thorny problems on the intersection of learning and games is the development of simple and practical algorithms that converge to Nash equilibria. The problem in its full generality is known to be intractable~\cite{daskalakis2006complexity,hart2003uncoupled}, however, recent developments in Machine Learning have led to a revived interest in the problem even in special classes of games. Unfortunately, the additional scrutiny has only helped crystallize the severity of the problem at hand through a diverse set of non-convergence, instability    
 results %for numerous standard learning dynamics 
 even in well motivated special classes of games~\cite{mertikopoulos2018cycles,bailey2019fast,flokas2020no,andrade2021learning,giannou21survival,letcher2021impossibility,bailey2018multiplicative,hsieh2021limits,bailey2020finitecolt,balduzzi2018mechanics}. Worse yet, standard online learning meta-algorithms, such as Multiplicative Weights Updates (MWU), have been shown to exhibit chaos~\cite{palaiopanos2017multiplicative,cheung2019vortices,cheung2020chaos,cheung2021chaos,bielawski2021follow,chotibut2019route, metaxas, bielawski2024memory}, which has been shown to be rather common in more complex games, e.g., as we increase the number of agents  ~\cite{GallaFarmer_PNAS2013,sanders2018prevalence,bielawski2021follow,chotibut2019route} and even in heterogenous settings \cite{bielawski2025heterogeneity}.
 Chaotic behavior has also been observed in auctions \cite{cheung3} and in dynamics induced by fictitious play learning rules \cite{sparrow,vanStrien}, as well as in discretized replicator dynamics \cite{mukhopadhyay,pandit,vilone}.
 Given this proliferation of negative results,
 %raises a tantalizing search for new ideas
 %Is there a promising path around such negative results? 
 %Given 
  what other approaches are left to explore? 
  
  
 An interesting hint can be found in some of the earliest AI work on the subject. \citep{singh2000nash} established arguably one of the first non-convergence results in the area, showing that gradient dynamics do not suffice to achieve point-wise convergence even in the trivial case of two agent, two strategy games. On the positive side, when those dynamics are non-convergent, time-average convergence results can be established.  Building up on their work, \citep{bowling2002multiagent} showed that a modification of these standard dynamics where the agents can dynamically update their step-size based on payoff cues from their environment suffices to stabilize these dynamics in all $2\times 2$ games. 
 Informally, the specific heuristic, Win or Learn Fast (WoLF), has the agents increase their learning rate when they are "losing" in an effort to escape from a non-promising region of the state space. Unfortunately, WoLF requires that each agent has knowledge of a Nash equilibrium strategy for themselves, which means it can only be applied in small games. On the positive side, this first result has led to several other similar heuristics, with promising results in small games~\cite{banerjee2003adaptive,bowling2004convergence,abdallah2008multiagent,kaisers2009evolutionary,leonardos2022exploration,bloembergen2015evolutionary}. While staying in the realm of small games, such heuristics have been shown to robustly improve the stability of other popular learning heuristics such as Proximal Policy Optimization \cite{schulman2017proximal,ratcliffe2019win}.
 On the negative side, even for slightly larger games most positive results are largely empirical in nature and effectively very little is known about the behavior of such techniques in games with many agents.
 %A further benefit of this approach is that is well supported by behavioral game theory \cite{camerer1998experience} and thus insights into such dynamics might also 
These works raise our key motivating question: 
\begin{quote}
\textit{Does the simple idea of judiciously increasing the learning rate to ``escape"  barren regions of the state space scale to games with a large number of agents? If not, what type of formal instability results can be established?}
\end{quote}
%\cite{singh2000nash}
%This proliferation of negative results, however, 
%\cite{gocke2002various,romero2015effect,} Path dependence.
%{%\color{blue}
% % It is easy to see that establishing  universal sweeping results for the chaotic or not behavior of non-autonomous dynamical systems appear to be intractable. 
% % To understand the fragility of the chaotic behavior in this setting, it suffices to take a sequence of maps where just a single rule that maps the whole strategy space to a fixed point eliminating by construction any chaotic behavior. Furthermore, it is mathematically unclear how we should quantify the long-term properties of a non-autonomous system, such as chaos, if the maps are ever-changing and never converge to a fixed system.'
 %Establishing a universal dichotomy between  chaotic and non-chaotic non-autonomous dynamical systems appears to be intractable. In this context, chaotic characterization is fragile; indeed a single rule in a sequence of maps that collapses the entire strategy space to a fixed point suffices to eliminate chaos. Furthermore, it is mathematically unclear how to quantify the long-term properties of a non-autonomous system, like chaos, when the maps are constantly changing and never converge to a fixed system.
% In general, providing such clear dichotomies what makes a non-autonomous system to be chaotic appears to be intractable. Indeed, chaotic behavior can be very fragile; even a single rule that maps the whole strategy space to a fixed point can eliminate chaos. In more general, quantifying the long-term properties of a system, like chaos is very challenging if the maps are ever-changing.

{\bf Our approach.} We focus on  one of the best-studied classes of large population games, non-atomic congestion games~\cite{roughgarden2002bad,Nisan:2007:AGT:1296179}
%\cite{roughgarden2004bounding}
where the agents learn using the ubiquitous MWU update rule~\cite{Arora05themultiplicative,freund1999adaptive,Littlestone:1994:WMA:184036.184040}. Furthermore, given the recent works of \cite{chotibut2019route,bielawski2021follow}, we focus on games with exactly two strategies/routes and linear cost functions, since such settings are already sufficiently hard for dynamics. Specifically, given fixed, non-adaptive learning rates, MWU dynamics typically will bifurcate to chaotic behavior for a large enough population size. Critically, however, these previous results are based on the celebrated "Period-3 implies chaos" methodology pioneered by Li--Yorke \cite{liyorke}, which is only applicable in autonomous, i.e., time-invariant systems. In contrast, understanding the emergent behavior in our case will require totally different techniques. 

Our model will allow for a wide range of dynamically adaptive learning rates. In particular, instead of having only two learning rates, fast and slow, as, e.g., in \citep{bowling2002multiagent}, we will allow for a continuous range of learning rates. Moreover,
the decision to increase/decrease the learning rate will be driven by a regret-like measure~\cite{shalev2011online}. Intuitively, each agent compares the historical time-average performance of both routes available to them.  If both routes appear very similar to each other then the agents favor large learning rates so as to reach sufficiently different configurations where they can hopefully find informative payoff signals to exploit. On the other hand, if one route is significantly better than the other then the agents will 
 %act more cautiously and 
take smaller but non-vanishing step sizes so as to take advantage of such opportunities without overcorrecting.   

%\cite{roughgarden2002bad}

%Despite the aforementioned difficulties, in this work we aim to provide a stepping stone result towards this direction. 
%Following the recent research line that focuses on congestion games, we investigate a class of game dynamics where agents can adapt their learning rate\footnote{!!Reference to dynamic adaptive old school methods} based on a notion of \emph{pseudo-regret}, which captures the adaptive nature of agents' strategy selection based on a summary of their historical payoffs. Critically, our update rule are not equivalent with any fixed MWU maps, in comparison with \cite{?}, since the learning rate varies among the iterations. Moreover, these systems cannot be considered one-dimensional, as they require maintaining both action probabilities and a past history summary. Consequently, previously established methods such as the celebrated 3-period characterization are not applicable in this context.

% all the until now described literature machinery can not be applied. More precisely, 3-period shortcut is not available.

% Building upon prior research on congestion games, we investigate a class of dynamics in which agents can adapt their learning rate based on the concept of pseudo-regret,  Importantly, our systems are not equivalent to any fixed Multiplicative Weight Update (MWU) maps, as the learning rate varies across iterations. As a result, these systems cannot be one-dimensional, as they require maintaining both action probabilities and a summary. Therefore, the use of previously established literature and methods is not applicable. Specifically, the use of 3-period shortcuts is not feasible in this context.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{Figures/abc.png}
%     \caption{\color{red} By definition of perpetual property this task is trivial for systems with fixed learning rates, as we can simply use By definition of perpetual property this task is trivial for systems with fixed learning rates,  }
%     \label{fig:my_label}
% \end{figure}

\textbf{Our main result.} We prove that our class of dynamics  exhibits Li--Yorke chaotic behavior, implying the existence of an uncountable set of initial conditions 
that become ``scrambled" by the dynamics (Theorem~\ref{theorem:dynamic-li-yorke}). Formally, for any two initial conditions from this set, the trajectories of the game dynamics come arbitrarily close to each other and move away from each other infinitely often.

{\bf Our techniques.} Despite the intense recent interest in developing formal arguments about chaos in game settings~\cite{bielawski2021follow,chotibut2019route,leonardos2021dynamical,piliouras2022multi}
%\cite{bielawski2021follow,chotibut2019route,leonardos2021dynamical,cheung2021learningIJCAI,piliouras2022multi},  
proving chaos in non-autonomous dynamical systems is a challenging endeavor, as the departure from one-dimensional autonomous systems gives up many established equivalences among different notions of chaos, such as volume expansion, topological entropy, and arbitrarily long periodic points. 


% Let's not describe things that do not work. 
One possible approach to addressing this challenge would be to first establish that the sequence of employed maps converges uniformly to a fixed chaotic map, and then transfer the resulting scrambled set of the limit system to the non-autonomous one.  
%
%However, a key obstacle in implementing this proof strategy is that the MWU map can never be uniformly convergent over the entire strategy space $\mathcal{X}$, as at the boundary of the pure action space $\mathrm{bd}(\mathcal{X})$, the map has trivial fixed points, and our adaptive update rule will converge to different behavior than in the interior of the strategy space $\mathrm{int}(\mathcal{X})$ .

This idea has been formalized in the theory of non-autonomous discrete
dynamical systems~\cite{kolyada1996topological}: for a sequence of surjective
interval maps $f_n$ converging uniformly to $f$, Li--Yorke chaos of $f$ is
inherited by the non-autonomous system~\cite{stefankova2016inheriting}
(see also~\cite{canovas2011li}), although other notions of chaos need not
transfer~\cite{dvorakova2012chaos}. These results do not apply directly here:
the learning rate $a_n$ depends on the whole history of the orbit, and hence on
$x_0$, so the iteration is not driven by a fixed sequence of maps, and the
convergence $a_n \to a^\star$ is uniform only on compact subintervals of
$(0,1)$, not on $[0,1]$.

Although such properties are not true for our system, it suffices to use a slightly relaxed version of them. We
 establish uniform convergence guarantees for initialization sets that are confined to the interior of the strategy space (Lemma~\ref{lemma:dynamic-strong-convergence}), while tolerating the discrepancy between the varying-step and the corresponding MWU map in the limit. To confirm the existence of an uncountable scrambled set, we propose a novel connection between the behavior of MWU maps with varying learning rates and symbolic dynamics. Essentially, our proof strategy entails assigning every binary sequence to a different initialization such that scrambled binary strings correspond to scrambled initializations of our non-autonomous dynamical system (Proof of Theorem~\ref{theorem:dynamic-li-yorke}).


% dividing the strategy space into regions, each assigned with a unique symbol, and representing the time evolution of the system as a sequence of symbols, known as a symbolic orbit. In order to establish Li-Yorke chaotic behavior, we aim to demonstrate the existence of an uncountable set of symbolic orbits that exhibit highly unpredictable behavior, indicating the presence of a scrambled set.

% Having this restriction, our technique will aim to provide  uniform convergence guarantees for initialization sets that lie exclusively in the interior and tolerate the difference between the volume expansion behavior of the non-autonomous system and the limit one. Finally to establish the existence of an uncountable scrambled set, we describe a novel reduction between the behavior MWU maps with varying learning rate and symbolic dynamics. 
% In a high level, our proof strategy is to divide the phase space of the system into regions, each assigned with a unique symbol. Then, the time evolution of the system can be represented as a sequence of symbols, known as a symbolic orbit. Hence, in order to prove the Li-Yorke chaotic behaviour, we will prove the existence of an uncountable set of symbolic orbits which behave highly unpredictable suggesting the existence of a scrambled set.


% the infamous \citeauthor{sharkovskii}'s ordering and the celebrated \citeauthor{liyorke} theorem ``\emph{Period


% Next, we show that if the sequence of employed maps uniformly converge to a fixed chaotic map then a ``Proximity and Separation'' chaotic property can be transferred to the non-autonomous dynamical system (Theorem ??).


The first part of our analysis (Section~\ref{sec:fixed}) involves  enhancing previously existing results for the case of fixed learning rate dynamics. Specifically, we present an explicit construction of a \emph{perpetual set} $\mathcal{F}(a)$, i.e., a forward invariant set where our dynamical system is surjective, $f_{a}(\mathcal{F}(a))=\mathcal{F}(a)$, where $f_{a}$ represents the MWU system with fixed learning rate $a$. (Lemma~\ref{lemma:perpetual}). Next we further show that, even in the presence of agent volatility due to their high learning rates, if their initial strategies lie within the interior of the strategy space, their strategies will eventually be absorbed into the perpetual set we have constructed (Lemma~\ref{lemma:absorbption}).


In the case of fixed learning rate, we are able to quantify an even stronger volume expansion result. Specifically, we show that the image of any arbitrarily small neighborhood of the mixed equilibrium of our game will converge exactly to the perpetual set we have constructed (Theorem~\ref{thm:volume-expansion}).

% Turning our attention to the adaptively dynamic learning rate, we demonstrate that the construction of the perpetual set $\mathcal{F}(a)$ allows us to show that, despite the volatility of players due to potentially high learning rates, there exists a set $\Delta$ - the closure of all perpetual sets $\mathcal{F}(a_n)$ - to which the dynamics will eventually converge, provided the initialization set lies within the interior of the solution space (Lemma~\ref{?},\ref{?}). Furthermore, utilizing this construction, we show that the average regret-like concepts converge for nearly all initial conditions (Theorem/Lemma ??). 

Turning our attention to the adaptively dynamic learning rate (Section~\ref{sec:dynamic}), we show that thanks to $\mathcal{F}(a)$, while learning rate may vary over iterations and initializations, there exists a set $\Delta$ \textendash the closure of all perpetual sets $\mathcal{F}(a_n)$ \textendash to which our dynamics eventually will be absorbed (Lemmas~\ref{lemma:forward-dynamic},\ref{lemma:absorption-dynamic}), provided the initialization set lies in the interior of solution space. Leveraging this property, we show that despite the volatility due to agents employing potentially high learning rates, our average regret-like concepts converge for nearly all initial conditions (Lemmas \ref{ref:average},\ref{ref:uniform},\ref{ref:cesaro}). It is noteworthy that this result requires a substantial degree of additional  technicality in contrast to its analogue for the fixed rate regime \cite{chotibut2019route}. 

%Intuitively our last preliminary step for our re, it is necessary to show that
Before developing our machinery for the symbolic dynamics reduction in Section~\ref{sec:turbulence}, our proof strategy includes an additional step of demonstrating that our system does not collapse early in any fixed point or subspace of strategies that lacks volume expansion, as this would eliminate chaos. To achieve this, we rely on Theorem~\ref{theorem:dynamic-volume-expansion} which guarantees that almost all neighborhoods of mixed equilibrium will avoid this scenario by  volume expanding and approximately covering $\mathcal{F}(\displaystyle\lim_{n\to\infty}a_n)$.
Putting everything together our main result about chaotic limit behavior follows. Finally, in Section \ref{sec:sec 6} we discuss the attractors of the system and the asymptotic relationship between the adaptive and standard MWU algorithms. 

% It is interesting to notice that the technical inguinity which is necessary to utilize in contrast with the similar established in the literature result for the fixed rate regime.


% Our analysis starts by refining existing results for the case of fixed learning rate dynamics. 


% More interestingly, we are able to show that despite the volatility of players' due to their high learning rates, if their initial strategy belong to the interior of the strategy space, then eventually their strategy would be absorbed into this perpetual set.

% In other words, even if players are volatile employing high learning rates, there exists a set of initial conditions such that $f(\mathcal{F}(a))=\mathcal{F}(a)$, where $f$ is the class of the maps that we take under consideration.

%  enodescribing a forward invar


































% Our analysis starts by refining existing results for the case of fixed learning rate dynamics. Specifically, we show that despite the volatility of players employing high learning rates, regret-like concepts converge for nearly all initial conditions (Theorem/lemma ??). 
%Actually, this observation does not hold only for pure strategies of the game, indicating that
% However,
%there exist regions of initial conditions around the boundary of the state space where the convergence becomes arbitrarily slow. 

% Next, we show that if the sequence of employed maps uniformly converge to a fixed chaotic map then a ``Proximity and Separation'' chaotic property can be transferred to the non-autonomous dynamical system (Theorem ??).

%(intuiteve

% However, a key roadblock in applying this result is that the map can never be uniformly convergent in the whole strategy space $\mathcal{X}$ since at the boundary pure actions $\mathrm{bd}(\mathcal{X})$ are trivially fixed points where the time-average regret/performance analysis converges to different values than $\mathrm{int}(\mathcal{X})$. 
% The reasoning of our proof strategy is to sidestep this concern by showing that for a fixed high enough learning rate $a$ there is an sub-interval $\mathcal{X}_{\text{inside}}\subset \mathcal{X}$ such that the underlying dynamical system $f_{a}$ is surjective\footnote{ 
% A function $f:\mathcal{X}\to\mathcal{Y}$ is surjective
% (also known as surjection, or onto) if for every element $y_{out}\in \mathcal{Y}$ can be mapped from some element (not necessarily unique) $x_{in}$ so that $f(x_{in}) = y_{out}$. In other words, every element of the function's codomain is the image of at least one element of its domain.
% }, i.e., $f_{a}(\mathcal{X})=\mathcal{X}$. 
% In our case we can prove that for $f_{a}$ to be the MWU map with learning rate $a$ the interval $\mathcal{X}_{\text{inside}} = [\min_{x\in\mathcal{X}} f_{a}(x), \max_{x\in\mathcal{X}} f_{a}(x)]$ both surjectivity (Lemma ??) and uniform convergence (Lemma ??) holds. Secondly, we need to prove that for any learning rate $(a_n)$ chosen by our class of adaptive rules, there exist always a set of initial conditions in $I_n\subseteq \mathcal{X}$ that covers $\mathcal{X}_{\text{inside}}$, namely $\mathcal{X}_{\text{inside}}\subseteq f_{a_n}(I_n)$ (Lemma ??). To motivate further the necessity of this step, we have to dig into the proof of Li-Yorke chaos in both autonomous and non-autonomous case. 



% {\color{red}
% \bf Our experiments} 
%  To be expanded only if it is necessary. 
% %den to deixame oti to |f'|>1 lyapunov two period trajectory argument
% }

% Our core contribution is analyzing the behavior of the dynamic learning rate version of the MWU dynamics. Although one could translate our dynamics to an autonomous dynamical system in higher dimensions, the key tool for studying Li Yorke chaos, namely the period three theorem no longer applies in higher dimensional systems. In fact it is known that the varying definitions of chaos are no longer equivalent above a single dimension.  So answering which of the chaotic properties of the fixed learning rate dynamics carry over to ours, if any, is highly non obvious.



% Alternatively our system can be viewed as a non autonomous dynamical system of $x_0, $x_n$. 
% In literature of chaotic systems there is existing work on non autonomous dynamical systems under the property of uniformly converging maps showing some ``kiss and leave'' property. However, the nuance in our case is that the map is not uniformly converging in [0,1] because 0 or 1 are fixed points on the dynamics so the learning rate does not converge to g(0).
% While there is existing work on non autonomous dynamical systems for uniformly converging maps that shows that the kiss and leave property holds. The nuance in our case that the map is not uniformly converging in [0,1] because 0 or 1 are fixed points on the dynamics so the learning rate does not converge to g(0).
% The reasoning of our analysis is to sidestep this concern by proving that for fixed high enough learning rate $a$ there is an interval X inside (0,1) where f(X,a) = X
% In our case we can prove that X = [fmax(a), fmin(a)] (all new results from this point on)
% Inside this interval we have both surjectivity and uniform convergence
% Second we need to prove that we can eventually cover this X with initial conditions of the non autonomous dynamical system 
% In other words we need to prove that the dynamical system does not collapse early in any interval that exhbits no volume expansion
% This is again non trivial because this interval needs to be bounded away from 0 and 1
% Although it is clear that $b$ has some volume expansion (clearly it is unstable), it is unclear if it covers X
% Even though b is becoming more unstable as $a$ increases (f'(b) goes to -infinity), the region where f' < -1 goes to 0 exponentially quickly (remember the map converges to a step function)
% To sidestep this we show that trajectories starting close to b either do the required volume expansion or converge to two periods
% Finally we show that two periods also need to exhbit volume expansion by studying the evolution of two period points as $a \to \infty$

%Our analysis starts by refining existing results on the for the fixed learning rate regime. 


% % Interestingly, we prove that dynamical system is Li-Yorke chaotic. 
% Our result is based on the following observations:
% \begin{enumerate}
% \item Besides the players are volatile with high learning rates, The notion of pseudo-regret converge for almost all initializations.
% \item Li-yorke chaos is robust to small perturbations of the map. Specifically, for a sequence of surjective maps which uniformly converge to a chaotic map, we can prove that the corresponding non-autonomous system.

% The high level intuition behind this mathematical claim. 
% (estw ena fixed system. Xekinontas apo ena diastima kataligei sto full surjective set/volume expansion. Akoma ki an exw ena approximate map pou den kanei toso volume expand. An parw tin $f^2$ tote xreiazomai ligotero diastima gia ton idio ogko.)
% \item
% Major caveat with previous arguments is that the map needs to converge uniformly for this result to hold. however, as we approach to the pure strategies as initial configuration the notion of pseudo-regret
% corverge arbitrarily slow, making uc infeasible.
% \end{enumerate}








% Chaos kai unpredictability eiani lektikos akrovatismos
% Chaos is a concept of unpredictability
% What is the correct definition of unpredictable
% Control theory..knowing the current state and model, i know the next state
% Under other perspective 

% If we are restricted on 1-dimension, Li and Yorke simplified the questionary
% because all definitions collapse.

% Diaforetikes ennoies: volume expansion set, 2-period, turb Expande

% Trying to confines autonomous dynamical systems, everything is unclear.
% 3-period do not guarrantee chaos.
% And systems who are chaotic over one definition they are not over other definition.

% Ola ta proigoumena paper se chaos kai games einai periorismena se 1-dimension kai non-adaptive. Mi antiprosopeutiko tou true human behavior. A question remains

% <<Existing results is a happy mathematical coincidence, or it is an indication for something more broadly?>>
% And if it exists...what is it?


% Non-stationary systems can alternate continuous without pattern of behaviour.
% Such a general anaysis is difficult

% Full generality results the prob
% As Stepping stone MWU with learning rate me vasi to historical payoff

% 1) Why li-yorke chaos is robust behavior? if system uniformly converge chaos is retained. But UC is not ubiquituous in all spectrum of DS. Nevertheless, there exist a set of initialization in the interior, the map is surjective to itself. Etsi tha paroume ena upperbound sto rate sto convergence rate.
% Den petiomaste exw apo auto prin statheropoithei to systima

% Chaos can be destroyed if there is a map that collapse everything to something stable. Mexri na statheropoihthei average convergence rate...yparxei ena set sto opoio eventually tha xanakatalavoume auto to surjective set..

% 2) All trajectories have not quantitavely the same behavior. Unstable fixed points
% 3) Average rate convergence is not the same for initialization ()

% Fixed learning rate is studied...intuitevely and only for the sake of a quick introduction...math is difficult...to volume expansion ginetai mono xeirotero.
% To fixed learning rate is the best we can see (lower bound)




% It is an important problem

% It is an unsolved problem

% Our solution works


==> output/Body/Prelims.tex <==
%----------------------------------------------------------------------
%%% INTRODUCTION
%----------------------------------------------------------------------
% !TEX root = ../main_new.tex


% What should go in the perliminaries?
% What is an autonomous dynamical system
% What is a non-autonomous dynamical system
% Definition of Li Yorke chaos for non-autonomous dynamical systems
% Period three result
% Congestion games
% MWU map
% Our dynamics

% {\color{red}\textbf{Notation} Maybe describe some notation here?}

\subsection{Dynamical systems \& Li--Yorke chaos}
% What is an (autonomous/non-autonomous) dynamical system? What is a trajectory of an initialization?
A discrete autonomous $m$-dimensional dynamical system is described by an equation $x_{n+1} = f(x_n)$ for a function $f: \mathbb{R}^m \to \mathbb{R}^m$. In contrast a discrete $m$-dimensional non-autonomous dynamical system is described by an equation $x_{n+1} = f(x_n, n)$ for a function $f: \mathbb{R}^m \times \mathbb{N} \to \mathbb{R}^m$. In both of these cases we can view the $x_n(x_0)$ iterate as a function of the initialization $x_0$. We thus term the sequence $\{x_n(x_0) \}_{n \in \mathbb{N}}$ the orbit of the dynamical system of $x_0$.

\begin{definition}
 We call two initializations $p,q$ of a dynamical system \emph{scrambled} if $\limsup_{n \to \infty} \| x_n(p) - x_n(q)\| >0$ and $\liminf_{n \to \infty} \| x_n(p) - x_n(q)\| = 0$. Intuitively the orbits of $p,q$ continuously alternate between moving apart and arbitrarily close respectively. A set $S$ is scrambled if every pair $p, q \in S$ is scrambled. 
\end{definition}

Based on the concept of a scrambled set, we can define the topological notion of Li--Yorke chaos for both autonomous and non-autonomous dynamical systems.

\begin{definition}
An autonomous/non-autonomous dynamical system is called Li--Yorke chaotic if there is an uncountably infinite set $S$ that is scrambled. 
\end{definition}

A famous result for the case of one dimensional autonomous dynamical systems provides a simple and easily verified sufficient condition for chaos based on periodic orbits:
\begin{theorem}[\cite{liyorke}]\label{thm:Li-Yorke}
Let $J$ be an interval and $f: J \to J$ be a continuous map of a dynamical system. If $f$ has a period-3 orbit, then it is Li--Yorke chaotic. 
\end{theorem}
\subsection{Linear congestion games} In this work we consider the case of non-atomic two strategy linear congestion games. In a non-atomic congestion game, there is a continuum of agents each of which controls an infinitesimal fraction of the total flow $N$. In each iteration, a fraction of agents $x$ choose the first action and $1-x$ the second one, suffering costs $c_1(x) = \gamma N x$ and $c_2(1-x) = \delta_{\mathrm{cost}} N (1-x)$ respectively where $\gamma, \delta_{\mathrm{cost}} > 0$ are the linear cost coefficients of each action respectively. 

\subsection{Multiplicative Weights Update}
The dynamics of the MWU meta-algorithm correspond to an autonomous dynamical system. Given the common learning rate of all agents $\eta > 0$, the MWU update is as follows
\begin{align*}
    x_{n+1} = \frac{x_n e^{-\eta c_1(x_n)}}{x_n e^{-\eta c_1(x_n)} + (1-x_n) e^{-\eta c_2(1-x_n)}}
            = \frac{x_n}{x_n + (1-x_n) e^{-\eta (c_2(1-x_n) - c_1(x_n))}}
\end{align*}

We can further simplify the MWU update rule by making the following changes of variables
\begin{align*}
    a = \frac{N\eta}{\delta_{\mathrm{cost}} + \gamma} && b = \frac{\delta_{\mathrm{cost}}}{\delta_{\mathrm{cost}} + \gamma}
\end{align*}
where $a$ corresponds to a normalized learning rate that accounts for the scale of $c_1$ and $c_2$ and $(b, 1-b)$ is the Nash equilibrium of the game. The simplified update rule can be expressed via a parametric map $f$ over $a$ and $b$ that captures the whole class of games we are interested in
{\small
\begin{equation}\label{eq:transform}
    x_{n+1} = f(x_n, a, b) = \frac{x_n}{x_n + (1-x_{n}) \exp(a (x_n -b))}.
\end{equation}
}
When $a,b$  are fixed we may skip them from the notation of MWU map and use just $f(x)$.

\subsection{Dynamic Learning Rate Model}
\label{sec:dynamic_rate}
Here we extend the MWU meta-algorithm to adaptive learning rates $\eta$. The basis of our adapting dynamics is a notion of pseudo-regret that the agents suffer when choosing the first action over the second one. The definition captures the average difference of costs between the two actions weighted by the learning rate at each iteration $\eta_i$:
\begin{equation*}
    r_{n+1} = \frac{1}{n+1} \sum_{i=0}^n \eta_i  [c_1(x_i) - c_2(1-x_i)].
\end{equation*}
Based on this calculation of pseudo-regret, the agents may seek to adapt their learning rates $\eta_i$ in order to balance between exploration and exploitation. When $r_n$ is big then it is clear that one action dominates over the other so the agents  seek to move in the direction of improving costs but hopefully not too aggressively so as not to overshoot, akin to a gradient-like dynamics. 
%slow down learning to make extended use of this cost gap for more iterations.
In contrast, when $|r_n|$ is close to zero the average penalty of switching between actions is small since they suffer the same weighted cost in average. Thus there is an opportunity for the agents to increase their learning rate to encourage exploration while the cost differences are low.  To hedge between exploration and exploitation as above, agents can pick appropriate function $h:\mathbb{R}\to \mathbb{R}^+$ that peaks at $0$ and setting $\eta_n = h(r_n)$.

This dynamics of adapting $\eta_i$ to the pseudo-regret can be implemented as a 2-dimensional non-autonomous dynamical system with $x_n$ and $r_n$ as its state variables:
\begin{align}\label{eq:old-update}
    x_{n+1} = f\left(x_n, \frac{Nh(r_n)}{\gamma+\delta_{\mathrm{cost}}}, b \right) \quad
    r_{n+1} = \frac{nr_n + h(r_n)(c_1(x_n) - c_2(1-x_n))}{n+1}.
\end{align}
The system is non-autonomous in the 2-dimensional space as the update rule of $r_n$ depends on $n$. We can always view $d$-dimensional non-autonomous systems as autonomous systems in $d+1$ dimensions by treating $n$ as an additional dimension. However, this does not really simplify things as \cref{thm:Li-Yorke} does not apply beyond a single dimension.

For simplicity, we rewrite the dynamics in terms of the normalized learning rates $a_i$. Let $a_i$ be the normalized learning rates corresponding to $\eta_i$ based on \cref{eq:transform}. We can then rewrite $r_{n+1}$ as
\begin{equation*}
    r_{n+1} = \frac{1}{n+1} \sum_{i=0}^n a_i  [x_i-b].
\end{equation*}
Similarly, given that $\eta_i$ and $\alpha_i$ are equivalent up to game specific scale parameters, we can always find a $g$ such that $a_n = g(r_n)$ . Instead of working in terms of the cumbersome dynamical system update rule \cref{eq:old-update}, we will be performing our analysis in terms of these simpler equations
\begin{align*}
    x_{n+1} = f(x_n, a_n, b) &&
    a_{n+1} = g\left( \frac{\sum_{i=0}^n a_i(x_i - b)}{n+1}\right).
\end{align*}
In the following sections we will make some assumptions on $g$. We will choose $g$ to be a continuous function bounded in $[a_{\min}, a_{\max}] \subset \mathbb{R}^+$. We will also assume that the initialization $a_0$ is also a constant in $[a_{\min}, a_{\max}]$.

Throughout this work we will think of $x_n$ and $a_n$ as functions of the initialization $x_0, a_0$.
Thus, the complete notation of the $n$-th iterate would be $x_n(x_0,a_0)$ and $a_{n}(x_0,a_0)$, however, when it does not hinder understanding we will drop the explicit description of all the dependencies. 

% N [\delta_{\mathrm{cost}} (1- x) - \gamma x] = N [\delta_{\mathrm{cost}} - (\delta_{\mathrm{cost}} + \gamma) x]  = N/(\delta_{\mathrm{cost}}+\gamma) [p - x]
% (1-\epsilon)^t = exp(t \ln(1-e)

 


==> output/Body/Turbulence.tex <==
The roadmap of this section is our  construction of the turbulent sets and
their connection with the symbolic dynamics in order to prove Li--Yorke chaos in our non-autonomous dynamical system. It should be noticed that our novel approach is a major departure from the standard techniques of period-3 orbit arguments that have been extensively used in the case of fixed learning rates. We start with some useful definition for our reduction.

\begin{definition}[\cite{shi2006study}]
A continuous map $f:I\to I$ is called \emph{turbulent} if there exist compact subintervals $J,K$ with at most one common point such that $J\cup K\subseteq f(J)\cap f(K)$
Additionally, the map is called \emph{strictly turbulent} if the subintervals can be chosen to be disjoint. Finally, the corresponding sets $J,K$ are called turbulent sets.
\end{definition}

Delving into the proof of \cite{liyorke}, it becomes clear that the chaotic map $f(x,a,b)$ has a period-3 orbit that exists within the interior of $\mathcal{F}(a)$. We take advantage of this property to demonstrate that $f^2(\cdot,a,b)$ is in fact a strictly turbulent map.

% \begin{lemma}\label{lemma:turbulence}
% For every $b \in (0,1)$, $f^2(\cdot,a,b)$  is in fact a strict turbulent map for sufficiently large $a$, i.e., there exist closed and disjoint intervals $K_a$ and $J_a$ in the interior of $\mathcal{F}(a)$ such that
% $f^2(K_a, a, b)$ and $f^2(J_a, a, b)$ are neighborhoods of $K_a \cup J_a$.
% \end{lemma}

\Needspace{27\baselineskip}
\begin{lemma}\label{lemma:turbulence}
For every $b \in (0,1)$, there is a $u_b$ such that for all $a> u_b$,  there exist closed and disjoint intervals $K_a$ and $J_a$ in the interior of $\mathcal{F}(a)$ such that
$f^2(K_a, a, b)$ and $f^2(J_a, a, b)$ are neighborhoods of $K_a \cup J_a$.
\end{lemma}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/plot_turb.pdf}
    \caption{Illustration of the turbulent sets described in Lemma \ref{lemma:turbulence}.}
    \label{fig:turbulence}
\end{figure}

\begin{proof}
As shown in Theorem \ref{theorem_turb_1} of Appendix \ref{app:turbulence}, if $b \in (0,1) \setminus \{\frac{1}{2}\}$ and for all $a>u_b$, the map $f(x,a,b)$ has a period-3 orbit in the interior of $\mathcal{F}(a)=[f_{\text{min}}(a), f_{\text{max}}(a)]$. This period-3 orbit has the form $f^2(x, a, b)< x< f(x, a, b) $ or its mirror image (See Theorem 1 in \cite{liyorke}). Without loss of generality, assume it has the form above. Then we can choose,
\begin{enumerate}
\item $d$  between $x$ and $f(x, a, b)$, so that $f(d,a, b)=x$ and hence $d<f^2(d,a, b)$. 
\item $z$ between $f(x)$ and $x$, so close that $f^2(z, a, b) >d$.
\item $q$ between $z$ and $x$, so close to $x$ that $f^2(q, a, b) < z$.
\item $c$ between $x$ and $d$, so close to $x$ that $f^2(c, a, b) < z$.
\end{enumerate} 
 Then, $J_a = [z,q]$ and $K_a = [c,d]$ are disjoint and
    \[  [z,d] \subset [f^2(q, a, b),f^2(z, a, b)] \subset  f^2(J_a),
        [z,d] \subset [f^2(c, a, b),f^2(d, a, b)] \subset  f^2(K_a)\]
Observe that $f^2(K_a, a, b)$ and $f^2(J_a, a, b)$ are supersets of $K_a$ and $J_a$ that share no endpoints with $K_a$ and $J_a$ so they are neighborhoods of $K_a \cup J_a$. Also since $x$, $f(x, a, b)$ and $f^2(x, a, b)$ are in the interior of the interval $[f_{\min}(a), f_{\max}(a)]$, we have that $J_a$ and $K_a$ have this property as well.
\end{proof}



Fig. \ref{fig:turbulence} illustrates two sets as described in Lemma \ref{lemma:turbulence}, following the construction of the proof. We now examine the properties of a fixed learning rate MWU map and its ability to create exponential decaying volume (length) turbulent sets. Our analysis centers around the key observation that since $f^2(K_a)$ covers $K_a\cup J_a$, then there exist necessarily, by continuity of $f^2$, at least two distinct subintervals, $Z_1,Z_2$, within $K_a$ whose $f^2$-image is precisely $K_a$ and $J_a$, respectively. By repeatedly applying this principle, we demonstrate that the $f^4$-image of these subintervals cover again $K_a\cup J_a$, and through induction, we can extend this property to higher compositions of $f$. 


\Needspace{28\baselineskip}
\begin{lemma}\label{lemma:turbulence-advanced}
For every $a > u_b$, there exist closed intervals $V_a^k \subseteq K_a$ and $U_a^k \subseteq J_a$ such that
\begin{align*}
    \lim_{k \to \infty} \text{diam}(V_a^k) = \lim_{k \to \infty} \text{diam}(U_a^k) = 0
\end{align*}
and for every $k \geq 0$ it holds that $f^{2k + 2}(V_a^k, a, b)$ and $f^{2k + 2}(U_a^k, a, b)$ are neighborhoods of $K_a \cup J_a$.
\end{lemma}

\begin{figure}[H]
    \centering

    % -------------------- (a) --------------------
    \begin{minipage}[c]{0.47\linewidth}
        \centering
        \resizebox{\linewidth}{!}{\input{Figures/tree.tex}}

        \vspace{2mm}
        {\small (a)}
    \end{minipage}
    \hfill
    % -------------------- (b) --------------------
    \begin{minipage}[c]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/plot_diam.pdf}

        \vspace{2mm}
        {\small (b)}
    \end{minipage}

    \caption{Illustration of the construction described in Lemma~\ref{lemma:turbulence-advanced}.}
    \label{fig:turbulence-advanced}
\end{figure}

\begin{proof}
We will prove the lemma by induction. Choosing $V_a^0 = K_a$ we know by Lemma~\ref{lemma:turbulence} that $f^2(V_a^0, a, b)$ is a neighborhood of $K_a \cup J_a$. Now let us assume that we have a $V_a^k \subseteq K_a$ such that $f^{2k + 2}(V_a^k, a, b)$ is a neighborhood of $K_a \cup J_a$. Since $K_a$ and $J_a$ are disjoint closed intervals , there are two disjoint closed intervals $Z_1$ and $Z_2$ of $V_a^k$ such that $f^{2k + 2}(Z_1, a, b)$ is a neighborhood of $K_a$ and $f^{2k + 2}(Z_2, a, b)$ is a neighborhood of $J_a$. As a result $f^{2k+4}(Z_1, a, b)$ and $f^{2k+4}(Z_2, a, b)$ are neighborhoods of $K_a \cup J_a$. Given that $Z_1$ and $Z_2$ are disjoint intervals of $V_a^k$ it must be the case that
\begin{equation*}
    \min\{\textrm{diam}(Z_1), \textrm{diam}(Z_2)\} \leq \textrm{diam}(V_a^k)/2.
\end{equation*}
We pick the interval with the smallest diameter as $V_a^{k+1}$ and thus 
\begin{equation*}
    0 \leq \textrm{diam}(V_a^k) \leq 2^{-k} \textrm{diam}(K_a) \implies \lim_{k \to \infty} \textrm{diam}(V_a^k) = 0.
\end{equation*}
Choosing $U_a^0 = J_a$ we can follow the same arguments for the rest of the $U_a^k$.
\end{proof}


% \begin{lemma}\label{lemma:turbulence-advanced}
% For every $b \in (0,1)$, and sufficiently large step-size,\\ there exist closed intervals $V_a^k \subseteq K_a$ and $U_a^k \subseteq J_a$ such that
% \begin{align*}
%     \lim_{k \to \infty} \textrm{diam}(V_a^k) = \lim_{k \to \infty} \textrm{diam}(U_a^k) = 0
% \end{align*}
% and for every $k \geq 0$ it holds that $f^{2k + 2}(V_a^k, a, b)$ and $f^{2k + 2}(U_a^k, a, b)$ are neighborhoods of $K_a \cup J_a$.
% \end{lemma}



The following lemma plays  an essential role in our symbolic dynamic proof of the Li--Yorke chaotic behavior. It allows us to construct a scrambled set of initial conditions through a set of abstract symbolic orbits. An illustration based on the construction described in the proof is shown in Fig. \ref{fig:turbulence-advanced}.

On a technical level, we utilize a range of machinery developed in this paper to prove this lemma. Specifically, we use Theorem~\ref{theorem:dynamic-volume-expansion} to firstly describe turbulent sets $J_{a^\star}\cup K_{a^\star}$ that lie within the interior of $\mathcal{F}(a^\star)$ and, for small enough $\epsilon$, within $\mathcal{F}(a^\star-\epsilon)$, and secondly to ensure that the non-autonomous dynamical system covers $J_{a^\star}\cup K_{a^\star}$.
Furthermore, to extend the implication of Lemma~\ref{lemma:turbulence-advanced} for the turbulent map $f^2(\cdot,a^\star,b)$ to the non-autonomous system $x_n$ map for the sets $J_{a^\star},K_{a^\star}$, we employ the uniform convergence guarantee provided by Lemma~\ref{lemma:dynamic-strong-convergence}, which controls the discrepancy between $x_{n+2}(S)$ and $f^2(x_n(S),a^\star,b)$ for any subinterval $S$ of $J_{a^\star},K_{a^\star}$. 

Our approach to demonstrate the Li--Yorke chaotic behavior through symbolic dynamics is summarized in the following high-level steps: 
\begin{itemize}
\item 
Assume that we can construct an uncountable set $\mathcal{S}$ of scrambled infinite length binary sequences, i.e., 
 for every pair of sequences $\sigma,\tau \in \mathcal{S}$ there exist $(i)$ an infinite length subsequence $(k_i)_{i\in \mathbb{N}}$ where the two sequences differ, i.e., $\sigma_{k_i}\neq\tau_{k_i}$ and $(ii)$ an infinite length subsequence  $(\ell_i)_{i\in \mathbb{N}}$ where the two sequences are equal, i.e., $\sigma_{\ell_i}=\tau_{\ell_i}$.
 \item For each element of $\sigma\in \mathcal{S}$ we construct a sequence of sets $\mathcal{A}_\sigma=(A_i)_{i\in \mathbb{N}}$ as follows: If the $k$-th place element is $0$ we use $V_{a^\star}^k$, whereas if it is $1$ we pick $U_{a^\star}^k$. We now apply Lemma~\ref{lemma:tracking} for each of the sequence of sets to get a corresponding initialization $x_0^{\sigma}$. We call this set of initializations $Q$.
 \item Since every pair of strings $\sigma,\tau$ is scrambled, we know that we can construct two infinite subsequences $\mu, \; \nu$ such that $\{x_{n_i}(x_0^{\sigma}) : i\in\mu\}$, $\{x_{n_i}(x_0^{\tau}) : i\in\mu\}$ belong to the same turbulent sets and $\{x_{n_i}(x_0^{\sigma}) : i\in\nu\}$, $\{x_{n_i}(x_0^{\tau}) : i\in\nu\}$ belong to the disjoint turbulent ones. Therefore, we can show that for every pair $\sigma,\tau\in Q$: $
 (i) \liminf\|\{x_{n}(x_0^{\sigma})-x_{n}(x_0^{\tau})\}\|=0
 \quad (ii) \limsup\|\{x_{n}(x_0^{\sigma})-x_{n}(x_0^{\tau})\}\|>0
$
\end{itemize}



\Needspace{23\baselineskip}
\begin{lemma}[Tracking Lemma]\label{lemma:tracking}
If $b \in (0, 1) \setminus \{\frac{1}{2} \}$, there exists a $d_b$ such that if $a_{\min} > d_b$, we can construct an increasing sequence $n_i$ with the following properties. For every sequence of intervals $A_i$ with $A_i = V_{a^\star}^i$ or $A_i = U_{a^\star}^i$, there exists a $x_0 \in [0,1]$ such that for all $i \geq 0$ it holds that $x_{n_i}(x_0) \in A_i$. 
\end{lemma}

\begin{figure}[H]
    \centering
  \begin{subfigure}[b]{0.43\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/plot_symb_specific.pdf}
    \caption{}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.43\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/plot_diff.pdf}
    \caption{}
  \end{subfigure}
  \captionsetup{justification=justified,singlelinecheck=false}
  \caption{(a) Illustration of the tracking construction from Lemma~\ref{lemma:tracking}: two specific subsequences satisfy $x_{n_i} \in A_i$. (b)~The trajectories repeatedly approach one another and separate again, with \mbox{$\liminf |x_{n_i}(\mu)-x_{n_i}(\nu)|=0$ but $\limsup |x_{n_i}(\mu)-x_{n_i}(\nu)|>0$}. These limits illustrate the scrambled behavior used in the proof.}
\label{fig: lem12}
%\vspace*{12pt}
\end{figure}

\begin{proof}
By continuity of $f_{\min}$ and $f_{\max}$ we know that
\begin{equation*}
    \lim_{\epsilon \to 0} f_{\min}(a^\star - \epsilon) = f_{\min}(a^\star) \quad \lim_{\epsilon \to 0} f_{\max}(a^\star - \epsilon) = f_{\max}(a^\star) 
\end{equation*}
By Lemma~\ref{lemma:turbulence} we know that $K_{a^\star}$ and $J_{a^\star}$ are in the interior of $[f_{\min}(a^\star), f_{\max}(a^\star)]$. As a result there is a sufficiently small $\epsilon > 0$ such that both of the following properties hold
\begin{gather*}
    a^\star > a^\star - \epsilon > a_{\min} \\
    [f_{\min}(a^\star - \epsilon), f_{\max}(a^\star - \epsilon)] \supseteq K_{a^\star} \cup J_{a^\star} 
\end{gather*}
Let us pick any interval $[\gamma, \zeta]$ such that $\{b\} \subset [\gamma, \zeta] \subset (0,1)$. By Theorem~\ref{app:theorem:dynamic-volume-expansion} and for the aforementioned $\epsilon$, we know that there is a $n^*$ such that
\begin{equation*}
    \forall n \geq n^* : \quad x_n([\gamma, \zeta]) \supseteq  [f_{\min}(a^\star - \epsilon), f_{\max}(a^\star - \epsilon)] \supseteq K_{a^\star} \cup J_{a^\star}
\end{equation*}
We also know that for all $i \geq 0$, $f^{2i +2}(V_{a^\star}^i, a^\star, b)$ and $f^{2i +2}(U_{a^\star}^i, a^\star, b)$ are neighborhoods of $K_{a^\star} \cup J_{a^\star}$. Thus for each $i \geq 0$ there must be an $\epsilon_i > 0$ such that $f^{2i +2}(V_{a^\star}^i, a^\star, b)$ and $f^{2i +2}(U_{a^\star}^i, a^\star, b)$ are $\epsilon_i$ neighborhoods of $K_{a^\star} \cup J_{a^\star}$. By Lemma~\ref{lemma:dynamic-strong-convergence}, there is a sequence of $m_i$ such that for all $i \geq 0$
\begin{equation*}
    \forall n \geq m_i \quad \max_{x_0 \in [\gamma, \zeta]} \abs{x_{n+2i+2}(x_0) - f^{2i+2}(x_n(x_0), a^\star, b)} \leq \epsilon_i
\end{equation*}
We are now ready to construct the sequence $n_i$. We choose $n_0 = \max\{m_0, n^*\}$. For $n_i$ with $i \geq 1$, we choose the minimum number with the following properties
\begin{gather*}
    (n_{i} - n_{i-1} -2i) \mod 2 = 0 \\
    n_{i} \geq n_{i-1} +2i \quad  n_{i} \geq m_i
\end{gather*}
It now remains to construct the required $x_0 \in [0,1]$ for each potential sequence of $A_i$. Since $x_{n_0}([\gamma, \zeta])$ is a superset of the disjoint closed intervals $K_{a^\star}=V_{a^\star}^0$ and $J_{a^\star}=U_{a^\star}^0$ we know that there are closed minimal intervals $I_0$ and $I_1$ such that
\begin{equation*}
    x_{n_0}(I_0) = V_{a^\star}^0 \quad x_{n_0}(I_1) = U_{a^\star}^0 
\end{equation*}
Since $n_0 \geq m_0$ we know that
\begin{equation*}
    \max_{x_0 \in I_0} \abs{x_{n_0+2}(x_0) - f^{2}(x_{n_0}(x_0), a^\star, b)} \leq \epsilon_0
\end{equation*}
Given that $x_{n_0}(I_0) = V_{a^\star}^0$ and $f^2(V_{a^\star}^0, a^\star, b)$ is an $\epsilon_0$ neighborhood of $K_{a^\star} \cup J_{a^\star}$, we can infer that
\begin{equation*}
    x_{n_0+2}(I_0) \supseteq K_{a^\star} \cup J_{a^\star}
\end{equation*}
With a similar analysis we can prove that
\begin{equation*}
    x_{n_0+2}(I_1) \supseteq K_{a^\star} \cup J_{a^\star}
\end{equation*}
Following the same steps repeatedly we can prove for any $k>0$ that
\begin{equation*}
    x_{n_0+2k}(I_0) \supseteq K_{a^\star} \cup J_{a^\star} \quad x_{n_0+2k}(I_1) \supseteq K_{a^\star} \cup J_{a^\star}
\end{equation*}
Since $n_1 = n_0 + 2k$ for some $k>0$ we can directly infer that
\begin{equation*}
    x_{n_1}(I_0) \supseteq K_{a^\star} \cup J_{a^\star} \quad x_{n_1}(I_1) \supseteq K_{a^\star} \cup J_{a^\star}
\end{equation*}
Hence we can construct minimal closed intervals $I_{00},I_{01} \subset I_0$ and $I_{10},I_{11} \subset I_1$ such that
\begin{equation*}
    x_{n_1}(I_{00}) = V_{a^\star}^1 \quad x_{n_1}(I_{01}) = U_{a^\star}^1 \quad x_{n_1}(I_{10}) = V_{a^\star}^1 \quad x_{n_1}(I_{11}) = U_{a^\star}^1
\end{equation*}
By induction, for any binary sequence $c$ of length $i$ we can construct two minimal closed intervals $I_{c_0 \cdots c_{i-1}0}$ and $I_{c_0 \cdots c_{i-1}1}$ subsets of $I_{c_0 \cdots c_{i-1}}$ such that
\begin{equation*}
    x_{n_i}(I_{c_0 \cdots c_{i-1} 0}) = V_{a^\star}^i \quad x_{n_i}(I_{c_0 \cdots c_{i-1} 1}) = U_{a^\star}^i
\end{equation*}
Now for any sequence $A_i$ such that $A_i = V_{a^\star}^i$ or $A_i = U_{a^\star}^i$ we can construct the corresponding sequence $c_i$ that has $c_i=0$ when $A_i= V_{a^\star}^i$ and $c_i=1$ when $A_i= U_{a^\star}^i$. Let us define
\begin{equation*}
    I_{c} = \cap_{i=0}^\infty I_{c_0 \cdots c_i}
\end{equation*}
By Cantor's intersection theorem, $I_{c}$ is non empty. Any $x_0 \in I_{c}$ satisfies the requirements of the lemma
\begin{equation*}
    \forall i \geq 0 \quad x_0 \in I_{c_0 \cdots c_i} \implies \forall i \geq 0 \quad x_{n_i}(x_0) \in A_i
\end{equation*}
\end{proof}

It is important to note that Lemma~\ref{lemma:tracking} ensures the ability to construct the same sequence of $n_i$ for any distinct sequence of $A_i$. Fig. \ref{fig: lem12} shows the construction described in the proof. Formalizing the outlined proof sketch, our final result follows:


\begin{theorem}\label{theorem:dynamic-li-yorke}
If $b \in (0, 1) \setminus \{\frac{1}{2} \}$, there exists a $d_b$ such that if $a_{\min} > d_b$, the dynamics of Equation~\ref{eq:old-update} are Li--Yorke chaotic. 
\end{theorem}
\begin{proof}
We first prove that there is an uncountable set $S$ of infinite length binary sequences with the following property: For every pair of sequences $i,j \in S$ there is an infinite length subsequence where the two sequences differ, i.e., one of $i,j$ is $0$ and the other is $1$.

We first define the equivalence relation $R$ over infinite length binary sequence such that two binary sequences are equivalent if and only if they differ in finitely many places. The relation is clearly reflexive, a sequence differs with itself in $0$ places, it is by definition symmetric and it is transitive, if a sequence $i$ differs in $k$ places with sequence $j$ and $j$ differs in $m$ places with a sequence $t$ then $i$ and $t$ differ in up to $m+k$ places which is also finite. Thus we can partition all binary sequences in equivalence classes where all pairs of all elements in the same class differ in finite places.

We now prove that each equivalence class has countably infinite binary sequences. Let us pick an element $\sigma$ of the equivalence class. For each member of the equivalence class $w$ we can construct a finite subset of $\mathbb{N}$ by picking the indices where $\sigma_t \neq w_t$. Inversely, for each finite subset of $\mathbb{N}$ we can construct a member of the equivalence by flipping the corresponding indices of $\sigma$. Thus there is a bijection between the members of the equivalence class and the finite subsets of $\mathbb{N}$. Because the finite subsets of $\mathbb{N}$ are countably infinite, so is each equivalence class.   

This allows us to prove that the relation $R$ has uncountably infinite number of equivalence classes. We proceed by contradiction. If we had countably many equivalence classes each having countably many elements then all of the binary sequences would be countable which is false.

To construct $S$ we only need to pick one element from each equivalence class. Since each pair belongs in a different equivalent class then they differ in infinite number of places which forms an infinite length subsequence. The set $S$ is uncountable because there are uncountably many equivalence classes.

We now prove that there is an uncountable set $S'$ of infinite length binary sequences that has the following two properties: First, for every pair of sequences $i,j \in S'$ there is an infinite length subsequence where the two sequences differ, i.e., one of $i,j$ is $0$ and the other is $1$. Second, for every pair of sequences $i,j \in S'$ there is an infinite length subsequence where the two sequences are equal, i.e., they are either both $0$ or $1$.

The construction works as follows: For each element of $i \in S$ we construct a new sequence. In its even places the sequence is $0$ and in its odd places we use the elements of $i$. Clearly by construction $S'$ remains uncountable and satisfies the first property as we can pick the subsequences from the odd places. The second property also holds because all sequences have the same elements in the even places.

For each element of $S'$ we construct a sequence of sets $T$ as follows: If the $k$th place element is $0$ we use $V_{a^\star}^k$, whereas if it is $1$ we pick $U_{a^\star}^k$. We now apply Lemma~\ref{lemma:tracking} for each of the sequence of sets to get a corresponding initialization $x_0$ and a subsequence of iteration indices $n_i$. We call this set of initializations $Q$. By the construction in Lemma~\ref{lemma:tracking} all initializations use the same subsequence $n_i$.

Let us pick two initializations $\mu, \nu \in Q$. By the construction of $T$ and $S'$ we have the following: There is an infinite subsequence of $n_i$, which we call $h_t$, where $x_{n_{h_t}}(\mu) \in V_{a^\star}^{h_t}$ and $x_{n_{h_t}}(\nu) \in U_{a^\star}^{h_t}$ or vice versa. Because $V_{a^\star}^{h_t}$ and $U_{a^\star}^{h_t}$ are disjoint we have that there is an infinite subsequence where the trajectories of $\mu$ and $\nu$ are bounded away from each other. In other words, we have that
\begin{equation*}
    \limsup_{n\to \infty} |x_n(\mu) - x_n(\nu)| > 0
\end{equation*}
Again by construction of $T$ and $S'$ we also have that there is an infinite subsequence of $n_i$, which we call $f_t$ such that either $x_{n_{f_t}}(\mu) \in V_{a^\star}^{f_t}$ and $x_{n_{f_t}}(\nu) \in V_{a^\star}^{f_t}$ or $x_{n_{f_t}}(\mu) \in U_{a^\star}^{f_t}$ and $x_{n_{f_t}}(\nu) \in U_{a^\star}^{f_t}$. Thus we have that
\begin{equation*}
    \forall t\geq 0 : |x_{n_{f_t}}(\mu) - x_{n_{f_t}}(\nu)| \leq \max\{\textrm{diam}(U_{a^\star}^{f_t}), \textrm{diam}(V_{a^\star}^{f_t})\}
\end{equation*}
By Lemma~\ref{lemma:turbulence-advanced}, we have that the right hand side converges to $0$. As a result
\begin{equation*}
    \lim_{t \to \infty} |x_{n_{f_t}}(\mu) - x_{n_{f_t}}(\nu)|  = 0
\end{equation*}
which directly implies that
\begin{equation*}
    \liminf_{n \to \infty} |x_n(\mu) - x_n(\nu)|  = 0.
\end{equation*}
Technically our dynamics are expressed in terms of two state variables $x_n$ and $r_n$ so distances in orbits need to account for both dimensions. Because $r_n \to 0$ for all initializations $x_0 \in (0,1)$, in all cases above we have $\lim_{n \to \infty} |r_n(\mu) - r_n(\nu)| = 0$ so the distances in the limit are not affected by the $r_n$ dimension.  

Picking $\{ (x, r) : x \in Q \text{ and } r= 0 \}$ as our scrambled set, which is equivalent to choosing $a_0 = g(0)$ for all $x \in Q$, we show that our dynamic learning rate dynamics are Li--Yorke chaotic. 
\end{proof}



In this work we have focused on the dynamics of \cref{eq:old-update}. But our proof strategy can be readily generalized to any rule $a_n(\cdot)$ as long as it uniformly converges to a sufficiently high constant rate.
\begin{corollary}
Let $a_n(\cdot)$ be a sequence of maps uniformly converging in $[0,1]$ to $a^\star> d_b$. Then the resulting dynamic learning rate system is Li--Yorke chaotic.
\end{corollary}


==> output/Body/sec6.tex <==
\begin{figure}[t!]
    \centering
  \begin{subfigure}[b]{0.43\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/bifurcation_MLE_vlat_0.4.pdf}
    \caption{}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.43\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/vlat_multistability.pdf}
    \caption{}
  \end{subfigure}
  
  \begin{subfigure}[b]{0.7\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/basin_heatmap_vlat_0.4_20.85.pdf}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.43\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/blat_tr_chaos.pdf}
    \caption{}
  \end{subfigure}
  
  \caption{(a) Bifurcation diagram of \eqref{sys_example} for $b=0.4$, $\beta=0.01$, and $\Delta_a=a_c/4$. The alternation between regular and chaotic behavior is particularly notable, as is the coexistence of periodic and chaotic attractors. Orbits colored in blue correspond to regular behavior, characterized by a Lyapunov exponent associated with the strategy dynamics $\lambda_x<0$. Orbits colored in red correspond to chaotic behavior, with $\lambda_x\geq 10^{-2}$. (b) A periodic attractor coexisting with a chaotic attractor for $a_c=26.85$. (c) The basins of attraction of the two attractors shown in (b). (d) Transient chaos for $a_c=20.93$ and $x_0=0.795.$}
\label{bif1}
%\vspace*{12pt}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/Fancy.png}
  \caption{An assortment of bifurcation diagrams for different adaptive learning rate schemes. Larger volatility (larger limit step-size) leads to more prominently unpredictable, chaotic behavior (dense limit-sets for large fraction of the parameter space). 
  While the limit of the scheme becomes more volatile, the behavior of the dynamics tends to be more chaotic as mixed Nash equilibrium moves away from the boundaries.
  }
  \label{fancy}
\end{figure*}

%\input{Body/sec6.tex}
Theorem \ref{theorem:dynamic-li-yorke} establishes the existence of an invariant chaotic set in the sense of Li--Yorke for the adaptive learning map \eqref{eq:old-update}, for any parameter $b\in(0,1)\setminus\{\frac{1}{2}\}$, provided that $a_{\text{min}}$ is sufficiently large. However, we stress that this chaotic set need not be attracting and may even coexist with a regular attractor, such as a periodic orbit. In case it is non-attracting, it frequently appears as a chaotic saddle and transient chaos is typically observed. As a result of the uniform convergence established in Lemma \ref{lemma:dynamic-strong-convergence}, it is natural to expect that for given values of $a^\star$ and $b$, the attractors of the adaptive system \eqref{eq:old-update} coincide with those of the standard MWU system with $a=a^\star$. Nevertheless, the adaptive learning rate may cause an orbit of \eqref{eq:old-update} to converge to a different attractor from that reached by the standard MWU system with $a=a^\star$ and the same initial condition, if multiple attractors coexist. In some cases, these two attractors may even be of completely different dynamical nature, for example, one periodic and the other chaotic. In fact, the potentially intricate structure of the basins of attraction may cause nearby initial conditions to converge to qualitatively different attractors. Consequently, an orbit of the adaptive system \eqref{eq:old-update} cannot, in general, be regarded simply as an orbit of the standard MWU rule with $a=a^\star$ and the same initial condition. 

To highlight the above points and illustrate the different dynamical regimes of \eqref{eq:old-update}, we consider the case where $g(r)=a_c-\Delta_a \tanh{ \left( \beta r \right) }$, which clearly satisfies the properties of Section \ref{sec:prelims} with $a_{\text{min}}=a_c-\Delta_a$ and $a_{\text{max}}=a_c+\Delta_a.$ As a result, the dynamical system reads
\begin{align}
x_{n+1}
&=
\frac{x_n}
{x_n+(1-x_n)\exp\!\left(a_n(x_n-b)\right)},\nonumber \\
a_{n+1}
&=
a_c-\Delta_a\,
\tanh\!\left[
\frac{\beta}{n+1}
\sum_{i=0}^{n}a_i(x_i-b)
\right]\nonumber,
\end{align}
\Needspace{9\baselineskip}
which can be rewritten as an autonomous system in the following form
\begin{align}
x_{n+1}
&=
\frac{x_n}
{x_n+(1-x_n)\exp\!\left(a_n(x_n-b)\right)},\nonumber \\
a_{n+1}
&=
a_c-\Delta_a\,
\tanh\!\left[
(1-s_n)
\operatorname{tanh}^{-1}\!\left(
\frac{a_c-a_n}{\Delta_a}
\right)
+\beta s_n a_n(x_n-b)
\right],\nonumber \\
s_{n+1}
&=
\frac{s_n}{1+s_n}. 
\label{sys_example}
\end{align}

In this case, we have $a_n\to a_c$. Let $b=0.4$, $\beta=0.01$, and $\Delta_a=a_c/4$. Figure \ref{bif1}(a) shows the bifurcation diagram of \eqref{sys_example} as $a_c$ varies. Orbits shown in blue correspond to regular behavior, characterized by a Lyapunov exponent associated with the strategy dynamics $\lambda_x<0$, whereas orbits shown in red correspond to chaotic behavior, with $\lambda_x\geq 10^{-2}$. For small values of $a_c$, the point $b$ is stable and subsequently loses stability through a period-doubling bifurcation. A cascade of period-doubling bifurcations then leads to the emergence of a chaotic attractor. Before this chaotic attractor is created, however, a distinct period-$4$ orbit is born through a saddle-node bifurcation and subsequently undergoes its own period-doubling cascade to chaos. The resulting chaotic attractor coexists with the periodic attractor, as shown in Fig.~\ref{bif1}(b). In fact, for the initial condition $x_0=0.2$, the orbit converges to the chaotic attractor under the adaptive system \eqref{sys_example}, whereas it converges to the periodic attractor under the standard MWU rule with $a=a_c$. Figure \ref{bif1}(c) shows the basins of attraction of the two attractors as a function of the initial condition $x_0$. The chaotic attractor illustrated in Fig.~\ref{bif1}(b) subsequently disappears through a crisis bifurcation, leaving the system with a single periodic attractor. As $a_c$ is increased further, the dynamics undergo additional bifurcations, giving rise to alternating periodic windows and chaotic regimes. Within the periodic windows the chaotic set survives as a chaotic saddle resulting in large chaotic intervals, i.e., the dynamics is transiently chaotic, as shown in Fig. \ref{bif1}(d).

Finally, to illustrate how these phenomena depend not only on the limiting learning rate $a^\star$ but also on the underlying game, i.e. on the parameter $b,$ Fig.~\ref{fancy} presents an assortment of bifurcation diagrams across different values of the equilibrium parameter $b$. Each colored sheet should be interpreted as a standard bifurcation diagram in which the limiting step size $a^\star$ is fixed, and $b$ is varied. As the limiting step size increases, increasingly complicated limit sets occupy a larger portion of the parameter range, with broad regions of apparently chaotic behavior. Moreover, for a fixed limiting step size, the dynamics generally become more intricate as the mixed Nash equilibrium moves away from the boundary of the strategy space. Thus, the bifurcation structure observed in Fig.~\ref{fancy} for the representative choice $b=0.4$ is not an isolated phenomenon, but is part of a richer organization of periodic and chaotic regimes across both the learning-rate and game parameters.







==> output/Figures/tree.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,445); %set diagram left start at 0, and has height of 445

%Straight Lines [id:da5394879690868122] 
\draw    (400.41,120.19) -- (220.22,120.63) ;
%Shape: Rectangle [id:dp22620449667588238] 
\draw   (353.11,80.07) .. controls (368.03,80.03) and (380.13,92.09) .. (380.16,107) -- (380.21,133.48) .. controls (380.23,148.39) and (368.17,160.51) .. (353.25,160.54) -- (267.52,160.75) .. controls (252.61,160.79) and (240.5,148.73) .. (240.47,133.82) -- (240.43,107.34) .. controls (240.4,92.43) and (252.47,80.31) .. (267.38,80.28) -- cycle ;
%Shape: Rectangle [id:dp7228055996711912] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.38 ] (350.15,93.6) .. controls (362.46,93.57) and (372.47,104.36) .. (372.49,117.7) .. controls (372.51,131.03) and (362.55,141.87) .. (350.23,141.9) .. controls (337.92,141.93) and (327.92,131.14) .. (327.89,117.8) .. controls (327.87,104.47) and (337.83,93.63) .. (350.15,93.6) -- cycle ;
%Shape: Rectangle [id:dp7805304186490449] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.54 ] (282.54,92.74) .. controls (295.65,92.71) and (306.31,104.41) .. (306.33,118.88) .. controls (306.36,133.34) and (295.75,145.09) .. (282.63,145.12) .. controls (269.51,145.16) and (258.86,133.46) .. (258.83,118.99) .. controls (258.81,104.53) and (269.42,92.78) .. (282.54,92.74) -- cycle ;
%Shape: Rectangle [id:dp26722576184194435] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.23 ] (296.78,115.49) -- (296.8,125.91) -- (282.26,125.94) -- (282.25,115.53) -- cycle ;
%Shape: Rectangle [id:dp7114197740947467] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.48 ] (276.3,115.65) -- (276.32,125.96) -- (264.42,125.99) -- (264.4,115.68) -- cycle ;
%Shape: Rectangle [id:dp28713158732908206] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.45 ] (365.91,115.33) -- (365.93,125.05) -- (355.41,125.08) -- (355.39,115.35) -- cycle ;
%Shape: Rectangle [id:dp7949640485877618] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.26 ] (347.73,115.48) -- (347.75,124.52) -- (333.55,124.55) -- (333.54,115.52) -- cycle ;
%Curve Lines [id:da6223172899952368] 
\draw    (323.42,214.36) .. controls (267.74,180.77) and (328.08,172.6) .. (341.46,124.52) ;
%Curve Lines [id:da85850722726211] 
\draw    (389.38,214.36) .. controls (428.78,175.68) and (380.81,182.8) .. (357.81,125.38) ;
%Straight Lines [id:da23292594611282658] 
\draw    (347.41,141.69) -- (347.41,198.11) ;
\draw [shift={(347.41,200.11)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp7163988727896183] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.38 ] (380.38,214.42) .. controls (392.89,214.39) and (403.05,219.15) .. (403.06,225.05) .. controls (403.07,230.95) and (392.94,235.75) .. (380.43,235.78) .. controls (367.91,235.8) and (357.76,231.04) .. (357.74,225.15) .. controls (357.73,219.25) and (367.86,214.45) .. (380.38,214.42) -- cycle ;
%Shape: Rectangle [id:dp0569652672292289] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.54 ] (320.97,214.87) .. controls (333.49,214.85) and (343.64,219.61) .. (343.66,225.51) .. controls (343.67,231.4) and (333.54,236.21) .. (321.02,236.23) .. controls (308.51,236.26) and (298.35,231.5) .. (298.34,225.6) .. controls (298.33,219.7) and (308.46,214.9) .. (320.97,214.87) -- cycle ;
%Shape: Rectangle [id:dp05967747812293944] 
\draw   (383.74,199.91) .. controls (398.65,199.88) and (410.77,210.79) .. (410.8,224.29) .. controls (410.83,237.78) and (398.76,248.74) .. (383.85,248.77) -- (317.87,248.91) .. controls (302.96,248.94) and (290.85,238.03) .. (290.82,224.54) .. controls (290.79,211.05) and (302.85,200.08) .. (317.76,200.05) -- cycle ;
%Straight Lines [id:da8214513088116734] 
\draw    (389.24,236.75) -- (413.36,300.02) ;
\draw [shift={(414.08,301.89)}, rotate = 249.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da26464971567954265] 
\draw    (311.14,234.75) -- (272.74,301.21) ;
\draw [shift={(271.74,302.95)}, rotate = 300.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp42175641186085866] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.38 ] (297.06,308.71) .. controls (305.88,308.69) and (313.04,312.32) .. (313.05,316.82) .. controls (313.06,321.32) and (305.91,324.98) .. (297.09,325) .. controls (288.27,325.02) and (281.11,321.39) .. (281.1,316.89) .. controls (281.09,312.4) and (288.23,308.73) .. (297.06,308.71) -- cycle ;
%Shape: Rectangle [id:dp032664278955003456] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.54 ] (247.14,308.82) .. controls (255.96,308.8) and (263.12,312.43) .. (263.13,316.93) .. controls (263.14,321.43) and (256,325.09) .. (247.17,325.11) .. controls (238.35,325.13) and (231.19,321.5) .. (231.18,317) .. controls (231.17,312.5) and (238.32,308.84) .. (247.14,308.82) -- cycle ;
%Shape: Rectangle [id:dp8818136761661548] 
\draw   (295.79,301.88) .. controls (310.7,301.84) and (322.8,308.2) .. (322.82,316.07) .. controls (322.84,323.94) and (310.76,330.34) .. (295.85,330.38) -- (252.44,330.47) .. controls (237.53,330.51) and (225.43,324.16) .. (225.41,316.29) .. controls (225.4,308.42) and (237.47,302.01) .. (252.38,301.98) -- cycle ;
%Shape: Rectangle [id:dp6116826652319777] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.38 ] (437.68,307.66) .. controls (446.5,307.64) and (453.66,311.27) .. (453.67,315.77) .. controls (453.68,320.27) and (446.54,323.93) .. (437.72,323.95) .. controls (428.89,323.97) and (421.74,320.34) .. (421.73,315.84) .. controls (421.72,311.34) and (428.86,307.68) .. (437.68,307.66) -- cycle ;
%Shape: Rectangle [id:dp6206250049588424] 
\draw  [fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.54 ] (387.77,307.77) .. controls (396.59,307.75) and (403.75,311.38) .. (403.76,315.87) .. controls (403.77,320.37) and (396.62,324.04) .. (387.8,324.06) .. controls (378.98,324.08) and (371.82,320.44) .. (371.81,315.95) .. controls (371.8,311.45) and (378.94,307.79) .. (387.77,307.77) -- cycle ;
%Shape: Rectangle [id:dp8474007656019541] 
\draw   (436.42,300.82) .. controls (451.33,300.79) and (463.43,307.14) .. (463.45,315.01) .. controls (463.46,322.88) and (451.39,329.29) .. (436.48,329.32) -- (393.07,329.42) .. controls (378.16,329.45) and (366.06,323.1) .. (366.04,315.23) .. controls (366.02,307.36) and (378.1,300.96) .. (393.01,300.92) -- cycle ;

% Text Node
\draw (380.4,225.1) node  [font=\footnotesize]  {$K_{a}$};
% Text Node
\draw (321,225.55) node  [font=\footnotesize]  {$J_{a}$};
% Text Node
\draw (297.05,258.69) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$f^{2}\left( V_{a}^{0} =K_{a} ,a,b\right)$};
% Text Node
\draw (370.6,334.16) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$f^{4}\left( V_{a}^{1} =Z_{2} ,a,b\right)$};
% Text Node
\draw (241.45,335.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$f^{4}( Z_{1} ,a,b)$};
% Text Node
\draw (267.29,191.53) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,rotate=-90.31]  {$\ddots $};
% Text Node
\draw (240.32,241.11) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,rotate=-89.16]  {$\ddots $};
% Text Node
\draw (218.72,156.67) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathcal{F}( a)$};
% Text Node
\draw (378.15,125.92) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$f_{\max}( a)$};
% Text Node
\draw (191.83,125.31) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$f_{\min}( a)$};
% Text Node
\draw (309.25,122.11) node [anchor=north west][inner sep=0.75pt]  [rotate=-358.71]  {$K_{a}$};
% Text Node
\draw (245.21,122.1) node [anchor=north west][inner sep=0.75pt]  [rotate=-358.71]  {$J_{a}$};
% Text Node
\draw (263.22,99.87) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\Xi _{1}$};
% Text Node
\draw (281.84,99.87) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\Xi _{2}$};
% Text Node
\draw (333.21,99.87) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$Z_{1}$};
% Text Node
\draw (350.71,99.87) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$Z_{2}$};
% Text Node
\draw (290.25,311.44) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$K_{a}$};
% Text Node
\draw (242.07,311.63) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$J_{a}$};
% Text Node
\draw (431.74,311.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$K_{a}$};
% Text Node
\draw (383.12,311.08) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$J_{a}$};


\end{tikzpicture}


==> output/Thanks.tex <==
%----------------------------------------------------------------------
%%% THANKS
%----------------------------------------------------------------------
% !TEX root = ./main_new.tex
%
%

Emmanouil V. Vlatakis-Gkaragkounis is grateful for financial support by the  Post-Doctoral FODSI-Simons Fellowship, Pancretan Association of America and Simons Collaboration on Algorithms and Geometry and Onassis Doctoral Fellowship. 
%This project was completed while he was a Post-Doctoral fellow at the Simons Institute for the Theory of Computing.
%\ackperiod
This research/project is also supported in part by the National Research Foundation, Singapore and DSO National Laboratories under its AI Singapore Program (AISG Award No: AISG2-RP-2020-016), NRF 2018 Fellowship NRF-NRFF2018-
07, NRF2019-NRF-ANR095 ALIAS grant, grant PIESGP-AI-2020-01, AME Programmatic Fund (Grant No.A20H6b0151) from the Agency for Science, Technology and Research (A*STAR) and Provost’s
Chair Professorship grant RGEPPV2101.\ackperiod


%
%PM is grateful for financial support by the French National Research Agency (ANR) in the framework of
%the ``Investissements d'avenir'' program (ANR-15-IDEX-02),
%the LabEx PERSYVAL (ANR-11-LABX-0025-01),
%MIAI@Grenoble Alpes (ANR-19-P3IA-0003),
%and the grant ALIAS (ANR-19-CE48-0018-01)

